Rewriting and Inductive Reasoning

Rewriting techniques based on reduction orderings generate "just enough" consequences to retain first-order completeness. This is ideal for superposition-based first-order theorem proving, but for at least one approach to inductive reasoning we show that we are missing crucial consequences. We therefore extend the superposition calculus with rewriting-based techniques to generate sufficient consequences for automating induction in saturation. When applying our work within the unit-equational fragment, our experiments with the theorem prover Vampire show significant improvements for inductive reasoning.

==> 6_related_work.tex <==

\paragraph{\bf Related Work.}
While auxiliary lemmas might be provided by users in an interactive theorem proving setting~\cite{IsabelleHol,sledgehammer}, the landscape of automated theorem proving does not support user guidance during proof search.
Fully-automatic approaches typically infer formulas equisatisfiable to a given conjecture (goal), then apply inductive reasoning to reduce them to subgoals.
These techniques include inductive generalizations~\cite{CADE19,CADE21,Aubin,Cruanes17}, using failed proof attempts \cite{Rippling93} and special sound inferences dealing with common patterns \cite{Wand17}. Our work extends these works by guiding proof search with auxiliary lemmas generated during proof search.

Lemma generation is exploited in theory exploration~\cite{HipSpec,ConjectureSynthesisForInductiveTheories}, with the aim to build a library of inductive lemmas for general usage. Such techniques do not guarantee relevance of generated lemmas with respect to a given conjecture. Our approach applies inductive inferences in such a way that this is not a concern.

The use of equational theories and term rewriting in inductive reasoning has already been investigated, the main difficulties being the lack of termination and confluence properties of general rewriting. Attempted solutions range from ensuring termination of function definitions~\cite{ACL2} and using completion procedures~\cite{ImplicitInductionInConditionalTheories,Rippling93} to interleaving heuristic rewriting with theorem proving~\cite{Wand17,FMCAD21}. Our work complements these approaches, by using rewriting-based equational reasoning for auxiliary lemma generation, and extending notions such as redundancy to applications of our induction rule. Our approach can be useful to non-equational fragments as well, using approaches to encode, for example, Horn formulas in equational logic~\cite{HornToEquational}.


==> misc.tex <==

\begin{mdframed}[frametitle={\colorbox{white}{\space \Calc{} (ground)\space}},
    innertopmargin=10pt,
    innerbottommargin=20pt,
    frametitleaboveskip=-\ht\strutbox,
    frametitlealignment=\center]

\begin{tabular}{p{.5\linewidth} p{.12\linewidth} l}
\multirow{2}{*}{
\AxiomC{$C\an{s[l]}\downarrow t$}
\AxiomC{$l\simeq r\lor D\downarrow t^\prime$}
\LeftLabel{(\DPar)}
\BinaryInfC{$C\an{s[r]}\lor D\downarrow s[l]$}
\DisplayProof}
&
\multirow{2}{*}{where}
& (1) $t^\prime\succeq l \succ r$,\\
& & (2) $t\succeq s[l]$.\\[2em]

\multirow{3}{*}{
\AxiomC{$C\an{s[r]}\updownarrow t$}
\AxiomC{$l\simeq r\lor D\updownarrow t^\prime$}
\LeftLabel{(\UPar)}
\BinaryInfC{$C\an{s[l]}\lor D\uparrow s[r]$}
\DisplayProof}
&
\multirow{3}{*}{where}
& (1) $l\succeq r$,\\
& & (2) $\updownarrow t^\prime=\ \downarrow t^\prime$ or $r\succeq t^\prime$,\\
& & (3) $\updownarrow t=\ \downarrow t$ or $s[r]\succeq t$.
\end{tabular}

\end{mdframed}


\begin{definition}
The \textit{rank} of a upward paramodulation inference $I$ in a derivation tree (denoted $r(I)$) is the number of forward paramodulation inferences on the path from $I$ to the root. The rank of a derivation tree $T$, denoted with $r(T)$, is the sum of ranks of all inferences in it. The number of \UPar inferences in a derivation tree $T$ we denote with $n(T)$.
\end{definition}

\begin{example}
    Show an example here.
\end{example}

\begin{lemma}\label{thm:rank0lemma}
Let $T$ be a ground derivation tree of \Par inferences on clauses with leaves $\mathcal{C}$ and root $C$. There exists a derivation tree $T^\prime$ with the same root and set of leaves with $r(T^\prime)=0$.
\end{lemma}
\begin{proof}
By transfinite induction on $n(T)\cdot\omega + r(T)$. If $n(T)=0$, then necessarily $r(T)=0$. If $r(T)=0$, the lemma trivially holds. Otherwise, let us assume that $n(T)>0$ and $r(T)>0$ and consider a upward paramodulation inference $I$ with a downward paramodulation inference $J$ as its parent. We denote the rest of their subtrees with $\dots$. Note that $r(I)\ge 1$.

In each case, we transform $T$ into a tree $T^\prime$ with the same root and leaves by changing $I$ and $J$ into $I^\prime$ and $J^\prime$ and moving subtrees. Either
\begin{itemize}
    \item[(*)] both $I^\prime$ and $J^\prime$ are downward paramodulation inferences in $T^\prime$ and $n(T)>n(T^\prime)$ or
    \item[(**)] $I^\prime$ is a downward paramodulation inference and $J^\prime$ is a upward paramodulation inference and we get $r(I)=r(J^\prime)+1$ and $r(J)=r(I^\prime)=0$, so $r(T)>r(T^\prime)$.
\end{itemize}
In both cases, the induction hypothesis applies to $T^\prime$ and it can be transformed into a tree $T^{\prime\prime}$ with $r(T^{\prime\prime})=0$.
Let $l\succ r$ and $u\succ w$.
% \noindent
% Let $\theta=\mgu(s,s^\prime)$ and $\mu=\mgu(l,l^\prime\theta)$, and $s\theta\not\succ t\theta$ and $r\mu\not\succeq l\mu$.
\medskip

\noindent
\textit{Case (1)} The conclusion of $I$ is the main premise of $J$.
\medskip

\noindent
\textit{Case (1.1)} The two term occurrences are in parallel positions in $C$.
\begin{center}
    % \def\defaultHypSeparation{\hskip 5pt}
    % \insertBetweenHyps{\hskip -4pt}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[r]}\an{t[u]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r \lor D$}
    \LeftLabel{$(I)$}
    \BinaryInfC{$C\an{s[l]}\an{t[u]}\lor D\uparrow s[r]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \RightLabel{$(J)$}
    \BinaryInfC{$C\an{s[l]}\an{t[w]}\lor D\lor D^\prime\downarrow t[u]$}
    \DisplayProof
\end{center}
The transformed tree $T^\prime$ is as follows. Since $I^\prime$ is a downward paramodulation and $J^\prime$ is an upward paramodulation, (**) applies.
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[r]}\an{t[u]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \LeftLabel{$(I^\prime)$}
    \BinaryInfC{$C\an{s[r]}\an{t[w]}\lor D^\prime\downarrow t[u]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r \lor D$}
    \RightLabel{$(J^\prime)$}
    \BinaryInfC{$C\an{s[l]}\an{t[w]}\lor D\lor D^\prime\uparrow s[r]$}
    \DisplayProof
\end{center}
%
\textit{Case (1.2)} One term occurrence is in $C$ and the other is in $D$.
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[r]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r \lor D\an{t[u]}$}
    \LeftLabel{$(I)$}
    \BinaryInfC{$C\an{s[l]}\lor D\an{t[u]}\uparrow s[r]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \RightLabel{$(J)$}
    \BinaryInfC{$C\an{s[l]}\lor D\an{t[w]}\lor D^\prime\downarrow t[u]$}
    \DisplayProof
\end{center}
Similarly, $I^\prime$ is a downward paramodulation and $J^\prime$ is an upward paramodulation, hence (**) applies to $T^\prime$, which is as follows.
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[r]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r \lor D\an{t[u]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \RightLabel{$(I^\prime)$}
    \BinaryInfC{$l\simeq r \lor D\an{t[w]}\lor D^\prime\downarrow t[u]$}
    \LeftLabel{$(J^\prime)$}
    \BinaryInfC{$C\an{s[l]}\lor D\an{t[w]}\lor D^\prime\uparrow s[r]$}
    \DisplayProof
\end{center}
\textit{Case (1.3)} The occurrence of $u$ is a subterm of $l$.
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[r]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l[u]\simeq r \lor D$}
    \LeftLabel{$(I)$}
    \BinaryInfC{$C\an{s[l[u]]}\lor D\uparrow s[r]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \RightLabel{$(J)$}
    \BinaryInfC{$C\an{s[l[w]]}\lor D\lor D^\prime\downarrow s[l[u]]$}
    \DisplayProof
\end{center}
If $r\succ l[w]$, then both $I^\prime$ and $J^\prime$ are downward paramodulations and (*) applies.
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[r]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l[u]\simeq r \lor D$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \RightLabel{$(I^\prime)$}
    \BinaryInfC{$l[w]\simeq r \lor D\lor D^\prime\downarrow l[u]$}
    \LeftLabel{$(J^\prime)$}
    \BinaryInfC{$C\an{s[l[w]]}\lor D\lor D^\prime\downarrow s[r]$}
    \DisplayProof
\end{center}
Otherwise, (**) applies.
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[r]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l[u]\simeq r \lor D$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \RightLabel{$(I^\prime)$}
    \BinaryInfC{$l[w]\simeq r \lor D\lor D^\prime\downarrow l[u]$}
    \LeftLabel{$(J^\prime)$}
    \BinaryInfC{$C\an{s[l[w]]}\lor D\lor D^\prime\uparrow s[r]$}
    \DisplayProof
\end{center}
\textit{Case (1.4)} The occurrence of $l$ is a strict subterm of $u$.
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[u[r]]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r \lor D$}
    \LeftLabel{$(I)$}
    \BinaryInfC{$C\an{s[u[l]]}\lor D\uparrow s[u[r]]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u[l]\simeq w\lor D^\prime$}
    \RightLabel{$(J)$}
    \BinaryInfC{$C\an{s[w]}\lor D\lor D^\prime\downarrow s[u[l]]$}
    \DisplayProof
\end{center}
If $u[r]\succ w$, then both $I^\prime$ and $J^\prime$ are downward paramodulations and (*) applies.
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[u[r]]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u[l]\simeq w\lor D^\prime$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r \lor D$}
    \RightLabel{$(I^\prime)$}
    \BinaryInfC{$u[r]\simeq w\lor D\lor D^\prime\downarrow u[l]$}
    \LeftLabel{$(J^\prime)$}
    \BinaryInfC{$C\an{s[w]}\lor D\lor D^\prime\downarrow s[u[r]]$}
    \DisplayProof
\end{center}
Otherwise, (**) applies.
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[u[r]]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u[l]\simeq w\lor D^\prime$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r \lor D$}
    \RightLabel{$(I^\prime)$}
    \BinaryInfC{$u[r]\simeq w\lor D\lor D^\prime\downarrow u[l]$}
    \LeftLabel{$(J^\prime)$}
    \BinaryInfC{$C\an{s[w]}\lor D\lor D^\prime\uparrow s[u[r]]$}
    \DisplayProof
\end{center}
\textit{Case (2)} The conclusion of $I$ is the side premise of $J$.\medskip

\noindent
\textit{Case (2.1)} The occurrence of $l$ is in $u$.
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[u[l]]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u[r]\simeq w\lor D^\prime$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r \lor D$}
    \RightLabel{$(I)$}
    \BinaryInfC{$u[l]\simeq w\lor D\lor D^\prime\uparrow u[r]$}
    \LeftLabel{$(J)$}
    \BinaryInfC{$C\an{s[r]}\lor D\lor D^\prime\downarrow s[u[l]]$}
    \DisplayProof
\end{center}
If $u[r]\succ w$, then both $I^\prime$ and $J^\prime$ are downward paramodulations and (*) applies.
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[u[l]]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r \lor D$}
    \LeftLabel{$(I^\prime)$}
    \BinaryInfC{$C\an{s[u[r]]}\lor D\downarrow s[u[l]]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u[r]\simeq w\lor D^\prime$}
    \RightLabel{$(J^\prime)$}
    \BinaryInfC{$C\an{s[w]}\lor D\lor D^\prime\downarrow s[u[r]]$}
    \DisplayProof
\end{center}
Otherwise, (**) applies.
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[u[l]]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r \lor D$}
    \LeftLabel{$(I^\prime)$}
    \BinaryInfC{$C\an{s[u[r]]}\lor D\downarrow s[u[l]]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u[r]\simeq w\lor D^\prime$}
    \RightLabel{$(J^\prime)$}
    \BinaryInfC{$C\an{s[w]}\lor D\lor D^\prime\uparrow s[u[r]]$}
    \DisplayProof
\end{center}
\textit{Case (2.2)} The occurrence of $l$ is in $w$.
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[u]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w[r]\lor D^\prime$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r \lor D$}
    \RightLabel{$(I)$}
    \BinaryInfC{$u\simeq w[l]\lor D\lor D^\prime\uparrow w[r]$}
    \LeftLabel{$(J)$}
    \BinaryInfC{$C\an{s[w[l]]}\lor D\lor D^\prime\downarrow s[u]$}
    \DisplayProof
\end{center}
Since $J^\prime$ is an upward paramodulation, (**) applies.
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[u]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w[r]\lor D^\prime$}
    \LeftLabel{$(I^\prime)$}
    \BinaryInfC{$C\an{s[w[r]]}\lor D^\prime\downarrow s[u]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D$}
    \RightLabel{$(J^\prime)$}
    \BinaryInfC{$C\an{s[w[l]]}\lor D\lor D^\prime\uparrow s[w[r]]$}
    \DisplayProof
\end{center}
\textit{Case (2.3)} The occurrence of $l$ is $D^\prime$.
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[u]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime\an{t[r]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r \lor D$}
    \RightLabel{$(I)$}
    \BinaryInfC{$l\simeq r\lor D\lor D^\prime\an{t[l]}\uparrow t[r]$}
    \LeftLabel{$(J)$}
    \BinaryInfC{$C\an{s[w]}\lor D\lor D^\prime\an{t[l]}\downarrow s[u]$}
    \DisplayProof
\end{center}
Since $J^\prime$ is an upward paramodulation, (**) applies.
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[u]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime\an{t[r]}$}
    \LeftLabel{$(I^\prime)$}
    \BinaryInfC{$C\an{s[w]}\lor D^\prime\an{t[r]}\downarrow s[u]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D$}
    \RightLabel{$(J^\prime)$}
    \BinaryInfC{$C\an{s[w]}\lor D\lor D^\prime\an{t[l]}\uparrow t[r]$}
    \DisplayProof
\end{center}
\qed
% \todo{Should we consider other inferences? Is this enough for equality reasoning?}

\end{proof}



\begin{lemma}\label{thm:switch-lemma}
Let $T$ be a ground derivation tree with leaves $\mathcal{C}$ and root $C$ such that all inferences are \ParC{} inferences and the only inference that violates \Calc{} restrictions is the inference at the root. There exists a derivation tree  $T^\prime$ corresponding to a derivation $\mathcal{C}\vdash_{\Calc} D$, such that:
\begin{itemize}
    \item if $C=C^\prime\downarrow s$, then either $D=C^\prime\downarrow t$ for some $t$ with $s\succeq t$ or $D=C^\prime\uparrow u$ for some $u$.
    \item if $C=C^\prime\uparrow s$, then $D=C^\prime\uparrow t$ for some $t$ with $s\succeq t$.
\end{itemize}
\end{lemma}

\begin{proof}
The proof is by induction on the size of the derivation tree. The base case is a tree with only one derivation and $l\succ r$ for which the claim is vacuously true since there cannot be any violated restriction of \Calc{}:
\begin{center}
    \AxiomC{$C\an{s[l]}$}
    \AxiomC{$l\simeq r\lor D$}
    \BinaryInfC{$C\an{s[r]}\lor D\downarrow s[l]$}
    \DisplayProof
    \qquad
    or
    \qquad
    \AxiomC{$C\an{s[r]}$}
    \AxiomC{$l\simeq r\lor D$}
    \BinaryInfC{$C\an{s[l]}\lor D\uparrow s[r]$}
    \DisplayProof
\end{center}
Consider a derivation tree with size $>1$. There are several cases to consider.

\noindent
(I) First, if the root is a downward paramodulation, we have the following:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l]}\updownarrow t$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\updownarrow t^\prime$}
    \BinaryInfC{$C\an{s[r]}\lor D\downarrow s[l]$}
    \DisplayProof
\end{center}
By assumption, one (or more) of the restrictions of \Calc{} is violated.

\noindent
\rule{\linewidth}{1pt}
(I.a) The first case is when $\updownarrow t^\prime=\downarrow t^\prime$, $\updownarrow t=\downarrow t$, $l\succ t^\prime$ and $t\succeq s[l]$. There are three subcases, the first is when the last paramodulation on the side premise paramodulated $t^\prime=l[u]$ into $l=l[w]$. This is impossible, since $l=l[w]\succ t^\prime=l[u]\succ l[w]$. The second case is when $t^\prime=r[u]$:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l]}\downarrow t$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r[u]\lor D$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$l\simeq r[w]\lor D\lor D^\prime\downarrow r[u]$}
    \BinaryInfC{$C\an{s[r[w]]}\lor D\lor D^\prime\downarrow s[l]$}
    \DisplayProof
\end{center}
By assumption $l\succ r[u]$, and we transform the tree as follows:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l]}\downarrow t$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r[u]\lor D$}
    \BinaryInfC{$C\an{s[r[u]]}\lor D\downarrow s[l]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$C\an{s[r[w]]}\lor D\lor D^\prime\downarrow s[r[u]]$}
    \DisplayProof
\end{center}
We can verify that the new tree is an \Calc{} derivation tree. The third subcase is when $t^\prime=t^\prime[u]$:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l]}\downarrow t$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\an{t^\prime[u]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$l\simeq r\lor D\an{t^\prime[w]}\lor D^\prime\downarrow t^\prime[u]$}
    \BinaryInfC{$C\an{s[r]}\lor D\an{t^\prime[w]}\lor D^\prime\downarrow s[l]$}
    \DisplayProof
\end{center}
The transformed tree is:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l]}\downarrow t$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\an{t^\prime[u]}$}
    \BinaryInfC{$C\an{s[r]}\lor D\an{t^\prime[u]}\downarrow s[l]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$C\an{s[r]}\lor D\an{t^\prime[w]}\lor D^\prime\downarrow t^\prime[u]$}
    \DisplayProof
\end{center}
We have to invoke the induction hypothesis on the tree of $C\an{s[r]}\lor D\an{t^\prime[u]}\downarrow s[l]$.

\noindent\rule{\linewidth}{1pt}
(I.b) $\updownarrow t^\prime=\downarrow t^\prime$, $\updownarrow t=\downarrow t$, $t^\prime\succeq l$ and $s[l]\succ t$. The last paramodulation in the main premise cannot have produced $s[l]$, that would contradict $s[l]\succ t$. The tree therefore looks like with $t=t[u]$:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l]}\an{t[u]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$C\an{s[l]}\an{t[w]}\lor D^\prime\downarrow t[u]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\downarrow t^\prime$}
    \BinaryInfC{$C\an{s[r]}\an{t[w]}\lor D\lor D^\prime\downarrow s[l]$}
    \DisplayProof
\end{center}
The transformed tree is as follows:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l]}\an{t[u]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\downarrow t^\prime$}
    \BinaryInfC{$C\an{s[r]}\an{t[u]}\lor D\downarrow s[l]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$C\an{s[r]}\an{t[w]}\lor D\lor D^\prime\downarrow t[u]$}
    \DisplayProof
\end{center}
\rule{\linewidth}{1pt}
(I.c) $\updownarrow t^\prime=\downarrow t^\prime$, $\updownarrow t=\downarrow t$, $l\succ t^\prime$ and $s[l]\succ t$. Similarly to (I.a) and (I.b), there are two subcases. The first is when $t=t[u]$ and $t^\prime=r[u^\prime]$:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l]}\an{t[u]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor C^\prime$}
    \BinaryInfC{$C\an{s[l]}\an{t[w]}\lor C^\prime\downarrow t[u]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r[u^\prime]\lor D$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u^\prime\simeq w^\prime\lor D^\prime$}
    \BinaryInfC{$l\simeq r[w^\prime]\lor D\lor D^\prime\downarrow r[u^\prime]$}
    \BinaryInfC{$C\an{s[r[w^\prime]]}\an{t[w]}\lor C^\prime\lor D\lor D^\prime\downarrow s[l]$}
    \DisplayProof
\end{center}
By assumption $l\succ r[u^\prime]$. If $s[r[u^\prime]]\succ t[u]$, then we transform the tree as follows:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l]}\an{t[u]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r[u^\prime]\lor D$}
    \BinaryInfC{$C\an{s[r[u^\prime]]}\an{t[u]}\lor D\downarrow s[l]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u^\prime\simeq w^\prime\lor D^\prime$}
    \BinaryInfC{$C\an{s[r[w^\prime]]}\an{t[u]}\lor D\lor D^\prime\downarrow s[r[u^\prime]]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor C^\prime$}
    \BinaryInfC{$C\an{s[r[w^\prime]]}\an{t[w]}\lor C^\prime\lor D\lor D^\prime\downarrow t[u]$}
    \DisplayProof
\end{center}
Otherwise, we obtain
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l]}\an{t[u]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r[u^\prime]\lor D$}
    \BinaryInfC{$C\an{s[r[u^\prime]]}\an{t[u]}\lor D\downarrow s[l]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor C^\prime$}
    \BinaryInfC{$C\an{s[r[u^\prime]]}\an{t[w]}\lor C^\prime\lor D\downarrow t[u]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u^\prime\simeq w^\prime\lor D^\prime$}
    \BinaryInfC{$C\an{s[r[w^\prime]]}\an{t[w]}\lor C^\prime\lor D\lor D^\prime\downarrow s[r[u^\prime]]$}
    \DisplayProof
\end{center}
The second subcase is done similarly.\todo{Detail second subcase.}

\noindent\rule{\linewidth}{1pt}
(I.d) $\updownarrow t^\prime=\uparrow t^\prime$, $\updownarrow t=\downarrow t$, $t\succeq s[l]$. There are three subcases. The first is when $t^\prime=l[w]$:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l[u]]}\downarrow t$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l[w]\simeq r\lor D$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$l[u]\simeq r\lor D\lor D^\prime\uparrow l[w]$}
    \BinaryInfC{$C\an{s[r]}\lor D\lor D^\prime\downarrow s[l[u]]$}
    \DisplayProof
\end{center}
If $l[w]\succ r$, we transform the tree as follows:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l[u]]}\downarrow t$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$C\an{s[l[w]]}\lor D^\prime\downarrow s[l[u]]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l[w]\simeq r\lor D$}
    \BinaryInfC{$C\an{s[r]}\lor D\lor D^\prime\downarrow s[l[w]]$}
    \DisplayProof
\end{center}
Otherwise:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l[u]]}\downarrow t$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$C\an{s[l[w]]}\lor D^\prime\downarrow s[l[u]]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l[w]\simeq r\lor D$}
    \BinaryInfC{$C\an{s[r]}\lor D\lor D^\prime\uparrow s[l[w]]$}
    \DisplayProof
\end{center}
The second is when $t^\prime=r[w]$:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l]}\downarrow t$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r[w]\lor D$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$l\simeq r[u]\lor D\lor D^\prime\uparrow r[w]$}
    \BinaryInfC{$C\an{s[r[u]]}\lor D\lor D^\prime\downarrow s[l]$}
    \DisplayProof
\end{center}
We have $l\succ r[u]\succeq r[w]$, and we transform the tree as follows:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l]}\downarrow t$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r[w]\lor D$}
    \BinaryInfC{$C\an{s[r[w]]}\lor D\downarrow s[l]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$C\an{s[r[u]]}\lor D\lor D^\prime\uparrow s[r[w]]$}
    \DisplayProof
\end{center}
The third subcase is when $t^\prime=t^\prime[w]$:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l]}\downarrow t$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\an{t^\prime[w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$l\simeq r\lor D\an{t^\prime[u]}\lor D^\prime\uparrow t^\prime[w]$}
    \BinaryInfC{$C\an{s[r]}\lor D\an{t^\prime[u]}\lor D^\prime\downarrow s[l]$}
    \DisplayProof
\end{center}
The transformed tree is:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l]}\downarrow t$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\an{t^\prime[w]}$}
    \BinaryInfC{$C\an{s[r]}\lor D\an{t^\prime[w]}\downarrow s[l]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$C\an{s[r]}\lor D\an{t^\prime[u]}\lor D^\prime\uparrow t^\prime[w]$}
    \DisplayProof
\end{center}
\rule{\linewidth}{1pt}
(I.e) $\updownarrow t^\prime=\uparrow t^\prime$, $\updownarrow t=\downarrow t$, $s[l]\succ t$. There are three subcases. The first is when $t=t[u]$ and $t^\prime=l[w^\prime]$:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l[u^\prime]]}\an{t[u]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor C^\prime$}
    \BinaryInfC{$C\an{s[l[u^\prime]]}\an{t[w]}\lor C^\prime\downarrow t[u]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l[w^\prime]\simeq r\lor D$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u^\prime\simeq w^\prime\lor D^\prime$}
    \BinaryInfC{$l[u^\prime]\simeq r\lor D\lor D^\prime\uparrow l[w^\prime]$}
    \BinaryInfC{$C\an{s[r]}\an{t[w]}\lor C^\prime\lor D\lor D^\prime\downarrow s[l[u^\prime]]$}
    \DisplayProof
\end{center}
By assumption, $s[l[u^\prime]]\succ t=t[u]$. If $l[w^\prime]\succ r$ and $s[l[w^\prime]]\succ t[u]$, then:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l[u^\prime]]}\an{t[u]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u^\prime\simeq w^\prime\lor D^\prime$}
    \BinaryInfC{$C\an{s[l[w^\prime]]}\an{t[u]}\lor D^\prime\downarrow s[l[u^\prime]]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l[w^\prime]\simeq r\lor D$}
    \BinaryInfC{$C\an{s[r]}\an{t[u]}\lor D^\prime\lor D\downarrow s[l[w^\prime]]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor C^\prime$}
    \BinaryInfC{$C\an{s[r]}\an{t[w]}\lor C^\prime\lor D\lor D^\prime\downarrow t[u]$}
    \DisplayProof
\end{center}
If $l[w^\prime]\succ r$ and $t[u]\succeq s[l[w^\prime]]$, then:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l[u^\prime]]}\an{t[u]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u^\prime\simeq w^\prime\lor D^\prime$}
    \BinaryInfC{$C\an{s[l[w^\prime]]}\an{t[u]}\lor D^\prime\downarrow s[l[u^\prime]]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor C^\prime$}
    \BinaryInfC{$C\an{s[l[w^\prime]]}\an{t[w]}\lor C^\prime\lor D^\prime\downarrow t[u]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l[w^\prime]\simeq r\lor D$}
    \BinaryInfC{$C\an{s[r]}\an{t[w]}\lor C^\prime\lor D\lor D^\prime\downarrow s[l[w^\prime]]$}
    \DisplayProof
\end{center}
Otherwise:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l[u^\prime]]}\an{t[u]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u^\prime\simeq w^\prime\lor D^\prime$}
    \BinaryInfC{$C\an{s[l[w^\prime]]}\an{t[u]}\lor D^\prime\downarrow s[l[u^\prime]]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor C^\prime$}
    \BinaryInfC{$C\an{s[l[w^\prime]]}\an{t[w]}\lor C^\prime\lor D^\prime\downarrow t[u]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l[w^\prime]\simeq r\lor D$}
    \BinaryInfC{$C\an{s[r]}\an{t[w]}\lor C^\prime\lor D\lor D^\prime\uparrow s[l[w^\prime]]$}
    \DisplayProof
\end{center}
The second case is when $t=t[u]$ and $t^\prime=r[w^\prime]$:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l]}\an{t[u]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor C^\prime$}
    \BinaryInfC{$C\an{s[l]}\an{t[w]}\lor C^\prime\downarrow t[u]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r[w^\prime]\lor D$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u^\prime\simeq w^\prime\lor D^\prime$}
    \BinaryInfC{$l\simeq r[u^\prime]\lor D\lor D^\prime\uparrow r[w^\prime]$}
    \BinaryInfC{$C\an{s[r[w^\prime]]}\an{t[w]}\lor C^\prime\lor D\lor D^\prime\downarrow s[l]$}
    \DisplayProof
\end{center}
By assumption $l\succ r[u^\prime]\succeq r[w^\prime]$. We transform the tree as follows:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l]}\an{t[w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r[w^\prime]\lor D$}
    \BinaryInfC{$C\an{s[r[w^\prime]]}\an{t[u]}\lor D\downarrow s[l]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor C^\prime$}
    \BinaryInfC{$C\an{s[r[w^\prime]]}\an{t[w]}\lor C^\prime\lor D\downarrow t[u]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u^\prime\simeq w^\prime\lor D^\prime$}
    \BinaryInfC{$C\an{s[r[u^\prime]]}\an{t[w]}\lor C^\prime\lor D\lor D^\prime\uparrow s[r[w^\prime]]$}
    \DisplayProof
\end{center}
The third subcase is done similarly.\todo{Detail third subcase.}

\noindent\rule{\linewidth}{1pt}
(I.f) $\updownarrow t^\prime=\downarrow t^\prime$, $\updownarrow t=\uparrow t$, $t^\prime\succeq l$. The first case is when the two rewrites are in different top-level terms but both originate from $C$. The tree looks as follows with $t=t[w]$:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l]}\an{t[w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$C\an{s[l]}\an{t[u]}\lor D^\prime\uparrow t[w]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\downarrow t^\prime$}
    \BinaryInfC{$C\an{s[r]}\an{t[u]}\lor D\lor D^\prime\downarrow s[l]$}
    \DisplayProof
\end{center}
The transformed tree is as follows:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l]}\an{t[w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\downarrow t^\prime$}
    \BinaryInfC{$C\an{s[r]}\an{t[w]}\lor D\downarrow s[l]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$C\an{s[r]}\an{t[u]}\lor D\lor D^\prime\uparrow t[w]$}
    \DisplayProof
\end{center}
The second subcase is when the second rewritten top-level term originates from the first side premise:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{t[w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime\an{s[l]}$}
    \BinaryInfC{$C\an{t[u]}\lor D^\prime\an{s[l]}\uparrow t[w]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\downarrow t^\prime$}
    \BinaryInfC{$C\an{t[u]}\lor D\lor D^\prime\an{s[r]}\downarrow s[l]$}
    \DisplayProof
\end{center}
The transformed tree is as follows:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{t[w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime\an{s[l]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\downarrow t^\prime$}
    \BinaryInfC{$u\simeq w\lor D^\prime\an{s[r]}\lor D\downarrow s[l]$}
    \BinaryInfC{$C\an{t[u]}\lor D\lor D^\prime\an{s[r]}\uparrow t[w]$}
    \DisplayProof
\end{center}
The third subcase is when the two paramodulated terms are in the same top-level term but in parallel positions:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l][w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$C\an{s[l][u]}\lor D^\prime\uparrow s[l][w]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\downarrow t^\prime$}
    \BinaryInfC{$C\an{s[r][u]}\lor D\lor D^\prime\downarrow s[l][u]$}
    \DisplayProof
\end{center}
The transformed tree is as follows:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l][w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\downarrow t^\prime$}
    \BinaryInfC{$C\an{s[r][w]}\lor D\downarrow s[l][w]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$C\an{s[r][u]}\lor D\lor D^\prime\uparrow s[r][w]$}
    \DisplayProof
\end{center}
The fourth subcase is when the downward paramodulated term is the subterm of the term that is upward paramodulated into:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u[l]\simeq w\lor D^\prime$}
    \BinaryInfC{$C\an{s[u[l]]}\lor D^\prime\uparrow s[w]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\downarrow t^\prime$}
    \BinaryInfC{$C\an{s[u[r]]}\lor D\lor D^\prime\downarrow s[u[l]]$}
    \DisplayProof
\end{center}
If $u[r]\succ w$, the transformed tree is as follows:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u[l]\simeq w\lor D^\prime$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\downarrow t^\prime$}
    \BinaryInfC{$u[r]\simeq w\lor D^\prime\downarrow u[l]$}
    \BinaryInfC{$C\an{s[u[r]]}\lor D\lor D^\prime\uparrow s[w]$}
    \DisplayProof
\end{center}
Otherwise:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u[l]\simeq w\lor D^\prime$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\downarrow t^\prime$}
    \BinaryInfC{$u[r]\simeq w\lor D^\prime\downarrow u[l]$}
    \BinaryInfC{$C\an{s[u[r]]}\lor D\lor D^\prime\downarrow s[w]$}
    \DisplayProof
\end{center}
The final, fifth subcase is when the downward paramodulated term is the strict superterm of the term that is upward paramodulated into:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l[w]]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$C\an{s[l[u]]}\lor D^\prime\uparrow s[l[w]]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l[u]\simeq r\lor D\downarrow t^\prime$}
    \BinaryInfC{$C\an{s[r]}\lor D\lor D^\prime\downarrow s[l[u]]$}
    \DisplayProof
\end{center}
If $l[w]\succ r$, the transformed tree is as follows:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l[w]]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l[u]\simeq r\lor D\downarrow t^\prime$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$l[w]\simeq r\lor D\downarrow l[u]$}
    \BinaryInfC{$C\an{s[r]}\lor D\lor D^\prime\downarrow s[l[w]]$}
    \DisplayProof
\end{center}
Otherwise:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l[w]]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l[u]\simeq r\lor D\downarrow t^\prime$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$l[w]\simeq r\lor D\downarrow l[u]$}
    \BinaryInfC{$C\an{s[r]}\lor D\lor D^\prime\uparrow s[l[w]]$}
    \DisplayProof
\end{center}
\rule{\linewidth}{1pt}
(I.g) $\updownarrow t^\prime=\downarrow t^\prime$, $\updownarrow t=\uparrow t$, $l\succ t^\prime$. The first case is when the two rewrites are in different top-level terms but both originate from $C$ and $t^\prime=r[u^\prime]$. The tree looks as follows with $t=t[w]$:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l]}\an{t[w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$C\an{s[l]}\an{t[u]}\lor D^\prime\uparrow t[w]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r[u^\prime]\lor D$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u^\prime\simeq w^\prime\lor C^\prime$}
    \BinaryInfC{$l\simeq r[w^\prime]\lor C^\prime\lor D\downarrow r[u^\prime]$}
    \BinaryInfC{$C\an{s[r[w^\prime]]}\an{t[u]}\lor C^\prime\lor D\lor D^\prime\downarrow s[l]$}
    \DisplayProof
\end{center}
Since $l\succ r[u^\prime]\succ r[w^\prime]$, the transformed tree is as follows:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l]}\an{t[w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r[u^\prime]\lor D$}
    \BinaryInfC{$C\an{s[r[u^\prime]]}\an{t[w]}\lor D\downarrow s[l]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u^\prime\simeq w^\prime\lor C^\prime$}
    \BinaryInfC{$C\an{s[r[w^\prime]]}\an{t[w]}\lor D\lor C^\prime\downarrow s[r[u^\prime]]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$C\an{s[r[w^\prime]]}\an{t[u]}\lor C^\prime\lor D\lor D^\prime\uparrow t[w]$}
    \DisplayProof
\end{center}
The second subcase is similar but $t^\prime=t^\prime[u^\prime]$ in a top-level term outside of $l\simeq r$.
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l]}\an{t[w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$C\an{s[l]}\an{t[u]}\lor D^\prime\uparrow t[w]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\an{t^\prime[u^\prime]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u^\prime\simeq w^\prime\lor C^\prime$}
    \BinaryInfC{$l\simeq r\lor C^\prime\lor D\an{t^\prime[w^\prime]}\downarrow t^\prime[u^\prime]$}
    \BinaryInfC{$C\an{s[r]}\an{t[u]}\lor C^\prime\lor D\an{t^\prime[w^\prime]}\lor D^\prime\downarrow s[l]$}
    \DisplayProof
\end{center}
The transformed tree is as follows:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l]}\an{t[w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\an{t^\prime[u^\prime]}$}
    \BinaryInfC{$C\an{s[r]}\an{t[w]}\lor D\an{t^\prime[u^\prime]}\downarrow s[l]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u^\prime\simeq w^\prime\lor C^\prime$}
    \BinaryInfC{$C\an{s[r]}\an{t[w]}\lor C^\prime\lor D\an{t^\prime[w^\prime]}\downarrow t^\prime[u^\prime]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$C\an{s[r]}\an{t[u]}\lor C^\prime\lor D\an{t^\prime[w^\prime]}\lor D^\prime\uparrow t[w]$}
    \DisplayProof
\end{center}
The third subcase is when the second rewritten top-level term originates from the first side premise and $t^\prime=r[u^\prime]$:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{t[w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime\an{s[l]}$}
    \BinaryInfC{$C\an{t[u]}\lor D^\prime\an{s[l]}\uparrow t[w]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r[u^\prime]\lor D$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u^\prime\simeq w^\prime\lor C^\prime$}
    \BinaryInfC{$l\simeq r[w^\prime]\lor C^\prime\lor D\downarrow r[u^\prime]$}
    \BinaryInfC{$C\an{t[u]}\lor C^\prime\lor D\lor D^\prime\an{s[r]}\downarrow s[l]$}
    \DisplayProof
\end{center}
The transformed tree is as follows:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{t[w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime\an{s[l]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r[u^\prime]\lor D$}
    \BinaryInfC{$u\simeq w\lor D\lor D^\prime\an{s[r[u^\prime]]}\downarrow s[l]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u^\prime\simeq w^\prime\lor C^\prime$}
    \BinaryInfC{$u\simeq w\lor C^\prime\lor D\lor D^\prime\an{s[r[w^\prime]]}\downarrow s[r[u^\prime]]$}
    \BinaryInfC{$C\an{t[u]}\lor C^\prime\lor D\lor D^\prime\an{s[r]}\uparrow t[w]$}
    \DisplayProof
\end{center}
The fourth subcase is similar, except $t^\prime=t^\prime[u^\prime]$ in a top-level term outside of $l\simeq r$.
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{t[w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime\an{s[l]}$}
    \BinaryInfC{$C\an{t[u]}\lor D^\prime\an{s[l]}\uparrow t[w]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\an{t^\prime[u^\prime]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u^\prime\simeq w^\prime\lor C^\prime$}
    \BinaryInfC{$l\simeq r\lor C^\prime\lor D\an{t^\prime[w^\prime]}\downarrow t^\prime[u^\prime]$}
    \BinaryInfC{$C\an{t[u]}\lor C^\prime\lor D\an{t^\prime[w^\prime]}\lor D^\prime\an{s[r]}\downarrow s[l]$}
    \DisplayProof
\end{center}
The transformed tree is as follows:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{t[w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime\an{s[l]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\an{t^\prime[u^\prime]}$}
    \BinaryInfC{$u\simeq w\lor D\an{t^\prime[u^\prime]}\lor D^\prime\an{s[r]}\downarrow s[l]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u^\prime\simeq w^\prime\lor C^\prime$}
    \BinaryInfC{$u\simeq w\lor C^\prime\lor D\an{t^\prime[w^\prime]}\lor D^\prime\an{s[r]}\downarrow t^\prime[u^\prime]$}
    \BinaryInfC{$C\an{t[u]}\lor C^\prime\lor D\an{t^\prime[w^\prime]}\lor D^\prime\an{s[r]}\uparrow t[w]$}
    \DisplayProof
\end{center}

\todo{Do the rest of these subcases}
The third subcase is when the two paramodulated terms are in the same top-level term but in parallel positions:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l][w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$C\an{s[l][u]}\lor D^\prime\uparrow s[l][w]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\downarrow t^\prime$}
    \BinaryInfC{$C\an{s[r][u]}\lor D\lor D^\prime\downarrow s[l][u]$}
    \DisplayProof
\end{center}
The transformed tree is as follows:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l][w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\downarrow t^\prime$}
    \BinaryInfC{$C\an{s[r][w]}\lor D\downarrow s[l][w]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$C\an{s[r][u]}\lor D\lor D^\prime\uparrow s[r][w]$}
    \DisplayProof
\end{center}
The fourth subcase is when the downward paramodulated term is the subterm of the term that is upward paramodulated into:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u[l]\simeq w\lor D^\prime$}
    \BinaryInfC{$C\an{s[u[l]]}\lor D^\prime\uparrow s[w]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\downarrow t^\prime$}
    \BinaryInfC{$C\an{s[u[r]]}\lor D\lor D^\prime\downarrow s[u[l]]$}
    \DisplayProof
\end{center}
If $u[r]\succ w$, the transformed tree is as follows:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u[l]\simeq w\lor D^\prime$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\downarrow t^\prime$}
    \BinaryInfC{$u[r]\simeq w\lor D^\prime\downarrow u[l]$}
    \BinaryInfC{$C\an{s[u[r]]}\lor D\lor D^\prime\uparrow s[w]$}
    \DisplayProof
\end{center}
Otherwise:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u[l]\simeq w\lor D^\prime$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\downarrow t^\prime$}
    \BinaryInfC{$u[r]\simeq w\lor D^\prime\downarrow u[l]$}
    \BinaryInfC{$C\an{s[u[r]]}\lor D\lor D^\prime\downarrow s[w]$}
    \DisplayProof
\end{center}
The final, fifth subcase is when the downward paramodulated term is the strict superterm of the term that is upward paramodulated into:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l[w]]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$C\an{s[l[u]]}\lor D^\prime\uparrow s[l[w]]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l[u]\simeq r\lor D\downarrow t^\prime$}
    \BinaryInfC{$C\an{s[r]}\lor D\lor D^\prime\downarrow s[l[u]]$}
    \DisplayProof
\end{center}
If $l[w]\succ r$, the transformed tree is as follows:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l[w]]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l[u]\simeq r\lor D\downarrow t^\prime$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$l[w]\simeq r\lor D\downarrow l[u]$}
    \BinaryInfC{$C\an{s[r]}\lor D\lor D^\prime\downarrow s[l[w]]$}
    \DisplayProof
\end{center}
Otherwise:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l[w]]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l[u]\simeq r\lor D\downarrow t^\prime$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$l[w]\simeq r\lor D\downarrow l[u]$}
    \BinaryInfC{$C\an{s[r]}\lor D\lor D^\prime\uparrow s[l[w]]$}
    \DisplayProof
\end{center}
\rule{\linewidth}{1pt}
(I.h) $\updownarrow t^\prime=\uparrow t^\prime$, $\updownarrow t=\uparrow t$\\
First subcase:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l]}\an{t[w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$C\an{s[l]}\an{t[u]}\lor D^\prime\uparrow t[w]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\an{t^\prime[w^\prime]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u^\prime\simeq w^\prime\lor C^\prime$}
    \BinaryInfC{$l\simeq r\lor C^\prime\lor D\an{t^\prime[u^\prime]}\uparrow t^\prime[w^\prime]$}
    \BinaryInfC{$C\an{s[r]}\an{t[u]}\lor C^\prime\lor D\an{t^\prime[u^\prime]}\lor D^\prime\downarrow s[l]$}
    \DisplayProof
\end{center}\todo{Finish this part.}
% Transformed:
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[l[u^\prime]]}\an{t[w]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w\lor D^\prime$}
%     \BinaryInfC{$C\an{s[l[u^\prime]]}\an{t[u]}\lor D^\prime\uparrow t[w]$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l[w^\prime]\simeq r\lor D$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u^\prime\simeq w^\prime\lor C^\prime$}
%     \BinaryInfC{$l[u^\prime]\simeq r\lor C^\prime\lor D\uparrow l[w^\prime]$}
%     \BinaryInfC{$C\an{s[r]}\lor C^\prime\lor D\lor D^\prime\downarrow s[l[u^\prime]]$}
%     \DisplayProof
% \end{center}
\rule{\linewidth}{1pt}
(II) If the root is an upward paramodulation, we have the following:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[r]}\updownarrow t$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\updownarrow t^\prime$}
    \BinaryInfC{$C\an{s[l]}\lor D\uparrow s[r]$}
    \DisplayProof
\end{center}
(II.a) If $\updownarrow t=\uparrow t$ and $t\succ s[r]$. The first case is when the paramodulations happen in the same top-level term, which together with $u\succ w$ yields $t=(s[r])[w]\succ (s[r])[u]\succ (s[r])[w]$, contradiction. The second case is when they are in different top-level terms and $t=t[w]$:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[r]}\an{t[w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$C\an{s[r]}\an{t[u]}\lor D^\prime\uparrow t[w]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\updownarrow t^\prime$}
    \BinaryInfC{$C\an{s[l]}\an{t[u]}\lor D^\prime\lor D\uparrow s[r]$}
    \DisplayProof
\end{center}
The transformed tree is as follows:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[r]}\an{t[w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\updownarrow t^\prime$}
    \BinaryInfC{$C\an{s[l]}\an{t[w]}\lor D\uparrow s[r]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w\lor D^\prime$}
    \BinaryInfC{$C\an{s[l]}\an{t[u]}\lor D^\prime\lor D\downarrow t[w]$}
    \DisplayProof
\end{center}

% \qed
\end{proof}


\redundancylemma*

\todo{Redundancy must be extended to equisatisfiable clause sets to make this lemma sensible.}
\begin{proof}
    By induction on $\succ$. First, note that if $r$ does not contain $t$, then $(L[l\mu\mapsto r\mu])[t\mapsto t^\prime]$ with $\mu=\theta\cdot\{x\mapsto t\}$ and $(L[t\mapsto t^\prime])[l\eta\mapsto r\eta]$ with $\eta=\theta\cdot\{x\mapsto t^\prime\}$ are the same.

    Since any clause resulting from \Ind with premise $L[t]\lor C$ inducting w.r.t. $t$ is of the form $\bigvee_{1\le i\le n}\widetilde{L}[t_i]\lor C$, we get the same clauses modulo some terms by first rewriting $l\eta$ into $r\eta$ with $\eta=\theta\cdot\{x\mapsto t\}$ in $L[t]\lor C$ and then performing an \Ind inference w.r.t. $t$ on the result, as by first performing an \Ind inference on $L[t]\lor C$ w.r.t. $t$ and then rewriting every occurrence of $l\mu$ in $L[t^\prime]$ with $\mu=\theta\cdot\{x\mapsto t^\prime\}$ in every resulting clause. The terms that these clauses differ on are fresh Skolem constants, therefore these two clause sets are equisatisfiable.

    TBD.\qed
\end{proof}


\section{Additional, not yet used stuff}

\subsection{Skipping \UPar inferences}

The primary goal of our calculus is to derive equational consequences of clauses that are easier to prove by induction. Additionally, as established in the previous section, the inductions that we can perform on such derived clauses is limited by redundancy criterion. However, some clauses derived by our calculus have no use for induction directly, because there is not a single induction based on them that is not redundant. Let us illustrate this with an example.

\begin{example}
Let us assume that we do not induct on non-recursive constructors alone, such as $\zero$ and $\nil$ because those cases can be usually solved without induction hypothesis. For any clause $L[t]\lor C$ that might be eligible to induction, axiom~\eqref{eq:app1} and \UPar gives an infinite chain of rewrites:
$$L[t]\lor C\rightsquigarrow L[\append(\nil,t)]\lor C\rightsquigarrow L[\append(\nil,\append(\nil,t))]\lor C\rightsquigarrow...$$

However, no matter how we induct on e.g. $L[\append(\nil,t)]\lor C$, either axiom~\eqref{eq:app1} make the result redundant or we get inductions that are duplicates of ones on $L[t]\lor C$. More specifically, as discussed above, we cannot induct on $\nil$. Moreover, Lemma~\ref{thm:redundancy-induction-lemma} and Lemma~\ref{above-position-lemma} disallow inducting on $t$ because of axiom~\eqref{eq:app1} or on $\append(\nil,t)$ or any term above it.\qed
\end{example}

\begin{definition}
We call a function \textit{useful for induction} if any ground instance of it can be inducted on. An equality $l\simeq r$ with $l\succ r$ is \textit{useful for induction} if there is a (possibly constant) term $f(\overline{t})\triangleleft l$ where $f$ is useful for induction.\footnote{Although the rule $\mathsf{Ind}$ uses all occurrences of the induction term $t$, for a rule that generalizes over occurrences, the equation $l\simeq r$ can be useful also when there are multiple occurrences of any variable in $l$.}
\end{definition}

\begin{lemma}
Any induction on the the rewritten literal of the conclusion of an \UPar inference is redundant if the the rewriting clause is a unit with an equation that is not useful for induction.
\end{lemma}
Unfortunately, even though a clause in itself is useless, it may be an intermediate clause needed to enable another \UPar inference. In general, we disallow \UPar inferences when the side premise $l\simeq r$ is not useful for induction. However, the following trick allows us to also derive useful clauses through intermediate useless clauses, without actually deriving the intermediate clauses.



We show an example of redundancy detection incorporated into our induction rules in the following variant of \Ind using the schema~\eqref{eq:list-schema} and the simplifying inference \NUDem.

\begin{mdframed}
\begin{tabular}{c p{.15\linewidth} p{.4\linewidth}}
\multirow{3}{*}{
\AxiomC{$\overline{L}\db{t} \lor C$}
\UnaryInfC{$\begin{matrix}\overline{L}\db{\nil}\lor L\db{\sigma_y} \lor C\\
\overline{L}\db{\nil}\lor \overline{L}\db{\cons(\sigma_x,\sigma_y)} \lor C\end{matrix}$}
\DisplayProof}
&\multirow{3}{*}{where}
& (1) $L\db{t}$ is ground,\\
& & (2) $\sigma_x$ and $\sigma_y$ are fresh constant symbols,\\
& & (3) there is no clause $l\simeq r$ and substitution $\theta$ s.t. (a) $l\theta\triangleleft L\db{x}$ and (b) $(l\succ r)\theta$ and (c) $t\not\trianglelefteq r$.
\end{tabular}
\end{mdframed}

The following lemma states that for any induction inference not performed due to restriction (2), there is an equisatisfiable induction inference which can be performed.

\begin{restatable}[]{lemma}{redundancylemma}
\label{thm:redundancy-induction-lemma}
Given two clauses $L\db{t}\lor C$ and $l\simeq r$ and a substitution $\theta$ s.t. $l\theta\triangleleft L\db{x}$, $(l\succ r)\theta$, $|\Sigma_\tau|>1$ where $t\in\tau$ and $t\not\trianglelefteq r$. The \Ind inference on $L\db{t}\lor C$ inducting w.r.t. $t$ is redundant.
\end{restatable}

Surely, using \UPar with a side premise that is non-unit is also possible, which leads to redundancies that cannot be detected with regular demodulation. However, we think that non-unit rewrites are often not that prevalent that using more expensive checks from e.g. subsumption demodulation would be worth using.\todo{prove that all inductions skipped by \mtt{IndR} are redundant.}



\begin{lemma}
    Given a clause set $\mathcal{C}$ with one goal clause $D$. If $\mathcal{C},D\vdash_{\Sup+\Calc{}+\Ind_G}\bot$, then $\mathcal{C},D\vdash_{\Sup+\Calc{}_{\bf G}+\Ind_G}\bot$.
\end{lemma}
\begin{proof}
    Let us consider a derivation tree from clauses $\mathcal{C}$ and goal clause $D$ obtained by $\Calc{}+\Ind_G$. If it is a $\Calc{}_{\bf G}+\Ind_G$ derivation tree, we are done. Otherwise, there is a \Calc{} inference performed on a non-goal clause.
\rule{\textwidth}{.2pt}
\noindent
\textbf{(I)} The lower one is a \DPar inference.\\
\noindent\rule{\textwidth}{.2pt}
\textbf{(I.a)} side condition: $l[u]\succeq l[w]$
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l[w]]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l[u]\simeq r\lor D$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w \lor D^\prime$}
    \BinaryInfC{$l[w]\simeq r\lor D\lor D^\prime\downarrow l[u]$}
    \BinaryInfC{$C\an{s[r]}\lor D\lor D^\prime\downarrow s[l[w]]$}
    \DisplayProof
\end{center}
{\color{red}{}This cannot be done as shown below the "multiset measure" increases.}
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l[w]]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w \lor D^\prime$}
    \BinaryInfC{$C\an{s[l[u]]}\lor D^\prime\uparrow s[l[w]]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l[u]\simeq r\lor D$}
    \BinaryInfC{$C\an{s[r]}\lor D\lor D^\prime\downarrow s[l[u]]$}
    \DisplayProof
\end{center}
{\color{red}{}Note: $l[u]\succ l[w]\succ r$}\\
\noindent\rule{\textwidth}{.2pt}
\textbf{(I.b)} side condition $r[u]\succeq l$ i.e. $r[u]\succ l$ in this case
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r[u]\lor D$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w \lor D^\prime$}
    \BinaryInfC{$l\simeq r[w]\lor D\lor D^\prime\downarrow r[u]$}
    \BinaryInfC{$C\an{s[r[w]]}\lor D\lor D^\prime\downarrow s[l]$}
    \DisplayProof
\end{center}
The transformed tree:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r[u]\lor D$}
    \BinaryInfC{$C\an{s[r[u]]}\lor D\uparrow s[l]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w \lor D^\prime$}
    \BinaryInfC{$C\an{s[r[w]]}\lor D\lor D^\prime\downarrow s[r[u]]$}
    \DisplayProof
\end{center}
{\color{red}{}$s[r[u]]\succ s[l]$ so the multiset measure increases.}\\
\rule{\textwidth}{.2pt}
\textbf{(I.c)}
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[l]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\an{t^\prime[u]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w \lor D$}
    \BinaryInfC{$l\simeq r\lor D\an{t^\prime[w]}\lor D^\prime\downarrow t^\prime[u]$}
    \BinaryInfC{$C\an{s[r]}\lor D\an{t^\prime[w]}\lor D^\prime\downarrow s[l]$}
    \DisplayProof
\end{center}
By assumption, $t^\prime[u]\succeq l$. This should be doable after the next induction. TBD.\\
\rule{\textwidth}{.2pt}
\noindent
\textbf{(II)} The lower one is an \UPar inference.\\
\noindent\rule{\textwidth}{.2pt}
\textbf{(II.a)}
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[r[w]]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r[u]\lor D$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w \lor D^\prime$}
    \BinaryInfC{$l\simeq r[w]\lor D\lor D^\prime\downarrow r[u]$}
    \BinaryInfC{$C\an{s[l]}\lor D\lor D^\prime\uparrow s[r[w]]$}
    \DisplayProof
\end{center}
{\color{red}{}If $r[u]\succ l\succ r[w]$, the measure increases so it cannot be done:}
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[r[w]]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w \lor D$}
    \BinaryInfC{$C\an{s[r[u]]}\lor D\uparrow s[r[w]]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r[u]\lor D^\prime$}
    \BinaryInfC{$C\an{s[l]}\lor D\lor D^\prime\downarrow s[r[u]]$}
    \DisplayProof
\end{center}
Otherwise, $l\succ r[u]\succ r[w]$ and the measure decreases.
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[r[w]]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w \lor D$}
    \BinaryInfC{$C\an{s[r[u]]}\lor D\uparrow s[r[w]]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r[u]\lor D^\prime$}
    \BinaryInfC{$C\an{s[l]}\lor D\lor D^\prime\uparrow s[r[u]]$}
    \DisplayProof
\end{center}
\noindent\rule{\textwidth}{.2pt}
\textbf{(II.b)}
Assume $l[u]\succ l[w]$ and $l[w]\succ r$
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[r]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l[u]\simeq r\lor D$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w \lor D^\prime$}
    \BinaryInfC{$l[w]\simeq r\lor D\lor D^\prime\downarrow l[u]$}
    \BinaryInfC{$C\an{s[l[w]]}\lor D\lor D^\prime\uparrow s[r]$}
    \DisplayProof
\end{center}
{\color{red}{}If $l[u]\succ l[w]\succ r$, the measure increases:}
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[r]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l[u]\simeq r\lor D$}
    \BinaryInfC{$C\an{s[l[u]]}\lor D\uparrow s[r]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w \lor D^\prime$}
    \BinaryInfC{$C\an{s[l[w]]}\lor D\lor D^\prime\downarrow s[l[u]]$}
    \DisplayProof
\end{center}
{\color{red}{}If $r\succ l[u]\succ l[w]$, this is not possible?}\\
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[r]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l[u]\simeq r\lor D$}
%     \BinaryInfC{$C\an{s[l[u]]}\lor D\downarrow s[r]$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w \lor D^\prime$}
%     \BinaryInfC{$C\an{s[l[w]]}\lor D\lor D^\prime\downarrow s[l[u]]$}
%     \DisplayProof
% \end{center}
% The transformed tree:
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[l]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l\simeq r[u]\lor D$}
%     \BinaryInfC{$C\an{s[r[u]]}\lor D\downarrow s[l]$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w \lor D^\prime$}
%     \BinaryInfC{$C\an{s[r[w]]}\lor D\lor D^\prime\downarrow s[r[u]]$}
%     \DisplayProof
% \end{center}
\rule{\textwidth}{.2pt}
\textbf{(II.c)}
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[r]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\an{t^\prime[u]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w \lor D$}
    \BinaryInfC{$l\simeq r\lor D\an{t^\prime[w]}\lor D^\prime\downarrow t^\prime[u]$}
    \BinaryInfC{$C\an{s[l]}\lor D\an{t^\prime[w]}\lor D^\prime\uparrow s[r]$}
    \DisplayProof
\end{center}
 This should be doable after the next induction. TBD.\\
\rule{\textwidth}{.2pt}
\textbf{(II.d)} side condition $s[r[u]]\succeq r[w]$
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[r[u]]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r[w]\lor D$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w \lor D^\prime$}
    \BinaryInfC{$l\simeq r[u]\lor D\lor D^\prime\uparrow r[w]$}
    \BinaryInfC{$C\an{s[l]}\lor D\lor D^\prime\uparrow s[r[u]]$}
    \DisplayProof
\end{center}
{\color{red}{}$l\succ r[u]\succ r[w]$. The measure increases (?):}
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[r[u]]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w \lor D^\prime$}
    \BinaryInfC{$C\an{s[r[w]]}\lor D^\prime\downarrow s[r[u]]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r[w]\lor D$}
    \BinaryInfC{$C\an{s[l]}\lor D^\prime\uparrow s[r[w]]$}
    \DisplayProof
\end{center}
\rule{\textwidth}{.2pt}
\textbf{(II.e)}
Assume $l[u]\succ r$. Side condition $s[r]\succeq l[w]$
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[r]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l[w]\simeq r\lor D$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w \lor D^\prime$}
    \BinaryInfC{$l[u]\simeq r\lor D\lor D^\prime\uparrow l[w]$}
    \BinaryInfC{$C\an{s[l[u]]}\lor D\lor D^\prime\uparrow s[r]$}
    \DisplayProof
\end{center}
If $l[u]\succ l[w]\succ r$, the measure decreases:
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[r]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l[w]\simeq r\lor D$}
    \BinaryInfC{$C\an{s[l[w]]}\lor D\uparrow s[r]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w \lor D^\prime$}
    \BinaryInfC{$C\an{s[l[u]]}\lor D\lor D^\prime\uparrow s[l[w]]$}
    \DisplayProof
\end{center}
{\color{red}{}Otherwise, $l[u]\succ r\succ l[w]$ and the measure increases?:}
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[r]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l[w]\simeq r\lor D$}
    \BinaryInfC{$C\an{s[l[w]]}\lor D\downarrow s[r]$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w \lor D^\prime$}
    \BinaryInfC{$C\an{s[l[u]]}\lor D\lor D^\prime\uparrow s[l[w]]$}
    \DisplayProof
\end{center}
TBD.\\
\rule{\textwidth}{.2pt}
\textbf{(II.f)}
\begin{center}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$C\an{s[r]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$l\simeq r\lor D\an{t^\prime[w]}$}
    \AxiomC{$\dots$}
    \noLine
    \UnaryInfC{$u\simeq w \lor D^\prime$}
    \BinaryInfC{$l\simeq r\lor D\an{t^\prime[u]}\lor D^\prime\uparrow t^\prime[w]$}
    \BinaryInfC{$C\an{s[l}\lor D\an{t^\prime[u]}\lor D^\prime\uparrow s[r]$}
    \DisplayProof
\end{center}
By assumption, $s[r]\succeq t^\prime[w]$. This should be doable after the next induction. TBD.

\begin{itemize}
    \item With \DPar:
    \begin{itemize}
        \item don't need to rewrite smaller side of equality (I.b)
        \item greater side needs rewriting when a \DPar is next
    \end{itemize}
    \item With \UPar:
    \begin{itemize}
        \item don't need to rewrite greater side of equality (II.e when $l[w]\succ r$)
    \end{itemize}
\end{itemize}
\end{proof}


\subsection{Redundant induction inferences}

As said earlier, \UPar inferences can result in redundant clauses and retaining these clauses seems very inefficient. As a remedy, in this section we show how to use this redundancy to skip \Ind inference applications on clauses resulting from \UPar. Let us first illustrate this idea on our running example.

\begin{example}\label{ex:simp}
Denote the left-hand side $\len(\append(\rev(\sigma_2),\cons(\sigma_1,\nil)))$ of the second literal of clause~\eqref{eq:indfconc1new2} with $t[s]$, where $s$ is one of its subterms except for $\sigma_1$\footnote{$\sigma_1$ is not of the sort $\lst$, so for clarity we do not consider inducting on it.}, $\sigma_2$ and $\rev(\sigma_2)$. Inducting with respect to $s$ in the literal $t[s]\not\simeq\suc(\len(\rev(\sigma_2)))$ of clause~\eqref{eq:indfconc1new2} with \Ind results in the clauses
% \begin{figure}
%     \centering
%     \tikz{
%     \node[](c1){$t[s]\not\simeq\suc(\len(\rev(\sigma_2)))$};
%     \node[right=of c1](c2){$\begin{aligned}
%         &t[\nil]\not\simeq\suc(\len(\rev(\sigma_2)))\lor t[\sigma_4]\simeq\suc(\len(\rev(\sigma_2)))\label{eq:redundant-clause1}\\
%         &t[\nil]\not\simeq\suc(\len(\rev(\sigma_2)))\lor t[\cons(\sigma_3,\sigma_4)]\not\simeq\suc(\len(\rev(\sigma_2)))\label{eq:redundant-clause2}
%     \end{aligned}$};
%     \node[below=of c1](c3){$t[s]\not\simeq\suc(\len(\sigma_2))$};
%     \node[below=of c2](c4){$\begin{aligned}
%         &t[\nil]\not\simeq\suc(\len(\sigma_2))\lor t[\sigma_4]\simeq\suc(\len(\sigma_2))\label{eq:equisat1}\\
%         &t[\nil]\not\simeq\suc(\len(\sigma_2))\lor t[\cons(\sigma_3,\sigma_4)]\not\simeq\suc(\len(\sigma_2))\label{eq:equisat2}
%     \end{aligned}$};
%     \node[below=of c2](c4){$\begin{aligned}
%         &t[\nil]\not\simeq\suc(\len(\sigma_2))\lor t[\sigma_4]\simeq\suc(\len(\sigma_2))\label{eq:equisat1}\\
%         &t[\nil]\not\simeq\suc(\len(\sigma_2))\lor t[\cons(\sigma_3,\sigma_4)]\not\simeq\suc(\len(\sigma_2))\label{eq:equisat2}
%     \end{aligned}$};
%     \draw[->] (c1) -- (c2) node[midway,above]{$\Ind$};
%     \draw[->] (c3) -- (c4) node[midway,above]{$\Ind$};
%     \draw[->] (c1) -- (c3) node[midway,left]{demodulates};
%     \draw[->] (c2) -- (c4) node[midway,right]{demodulates*};
%     % \draw[->] (c1) -- (c2);
%     }
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}
\begin{align}
    &t[\nil]\not\simeq\suc(\len(\rev(\sigma_2)))\lor t[\sigma_4]\simeq\suc(\len(\rev(\sigma_2)))\label{eq:redundant-clause1}\\
    &t[\nil]\not\simeq\suc(\len(\rev(\sigma_2)))\lor t[\cons(\sigma_3,\sigma_4)]\not\simeq\suc(\len(\rev(\sigma_2)))\label{eq:redundant-clause2}
\end{align}
%
where $\sigma_3$ and $\sigma_4$ are fresh constant symbols. Notice that $\len(\rev(\sigma_2))$ is present in all literals added by the \Ind inference in clauses~\eqref{eq:redundant-clause1} and \eqref{eq:redundant-clause2} and therefore (using $\succ$ from Example~\ref{ex:calc}) clause~\eqref{eq:conj-neg-hyp} can simplify these clauses by demodulating all such literals one-by-one to obtain:
\begin{align}
    &t[\nil]\not\simeq\suc(\len(\sigma_2))\lor t[\sigma_4]\simeq\suc(\len(\sigma_2))\label{eq:equisat1}\\
    &t[\nil]\not\simeq\suc(\len(\sigma_2))\lor t[\cons(\sigma_3,\sigma_4)]\not\simeq\suc(\len(\sigma_2))\label{eq:equisat2}
\end{align}
%
However, clauses~\eqref{eq:equisat1} and \eqref{eq:equisat2} are equisatisfiable to the clauses resulting from an \Ind inference on clause~\eqref{eq:indfconc1new1} with respect to the same term $s$, since the latter clause set has fresh constant symbols in place of $\sigma_3$ and $\sigma_4$. Therefore, none of the inductions on $s$ in the second literal of clause~\eqref{eq:indfconc1new2} need to be performed.
\qed
\end{example}

Redundant induction clauses like the ones shown in Example~\ref{ex:simp} cannot be dealt with effectively by the saturation algorithm for the following reasons:
\begin{enumerate}
    \item For a clause resulting from $n$ consecutive \UPar inferences, $\mathcal{O}(n)$ many simplifications may be needed after an \Ind inference is performed to get the equisatisfiable clause set.
    \item Since the \Ind inference often produces fresh constant symbols, instead of general subsumption, equisatisfiability w.r.t. these fresh symbols needs to be performed, which is much harder.
\end{enumerate}
%
An alternative is to recognize that the clauses from an \Ind inference will be redundant before they are generated.


% Alternative proof:
% \begin{proof}
% Take the multiset $M(T)$ of multisets of the ranks of inferences on each path from a leaf of $T$ to the root of $T$. The proof is by induction on $M(T)$ with the multiset order $(>_{mul})_{mul}$ denoted with $\sqsupset$ for clarity. The base case is when all multisets in $M(T)$ contain only zeros, when the property trivially holds. Otherwise, let us assume that $M(T)$ contains some multiset with non-zero values and a \UPar inference $I$ with $r(I)> 1$ s.t. its parent is an \DPar inference $J$ exists. The induction hypothesis is that the claim holds for all $T^\prime$ with $M(T)\sqsupset M(T^\prime)$. \todo{Make remark about removing duplicate literals}

% \noindent
% \textit{Case 1.1}: $p$ is parallel to all positions of $l$ or $l\trianglelefteq t$:
% \begin{prooftree}
%     \AxiomC{$(C[s]_p)[l]$}
%     \AxiomC{$(t\simeq s \lor D)[l]$}
%     \BinaryInfC{$(C[t]_p\lor D)[l]$}
%     \AxiomC{$l\simeq r\lor D^\prime$}
%     \BinaryInfC{$(C[t]_p\lor D)[r]\lor D^\prime$}
% \end{prooftree}
% If $t[r]\succeq s[r]$, the transformed tree is as follows:
% \begin{prooftree}
%     \AxiomC{$(C[s]_p)[l]$}
%     \AxiomC{$l\simeq r\lor D^\prime$}
%     \BinaryInfC{$(C[s]_p)[r]\lor D^\prime$}
%     \AxiomC{$(t\simeq s \lor D)[l]$}
%     \AxiomC{$l\simeq r\lor D^\prime$}
%     \BinaryInfC{$(t\simeq s \lor D)[r]\lor D^\prime$}
%     \BinaryInfC{$(C[t]_p\lor D)[r]\lor D^\prime$}
% \end{prooftree}
% The multisets in $M(T)$ corresponding to branches involving $(C[s]_p)[l]$ to a branch outside of the shown part has the same multiplicity as in $M(T)$. The paths corresponding to Otherwise $t[r]\prec s[r]$ and we may need to fix the conclusion of the second inference by adding a chain of \UPar inferences:
% \begin{prooftree}
%     \AxiomC{$(C[s]_p)[l]$}
%     \AxiomC{$l\simeq r\lor D^\prime$}
%     \BinaryInfC{$(C[s]_p)[r]\lor D^\prime$}
%     \AxiomC{$(t\simeq s \lor D)[l]$}
%     \AxiomC{$l\simeq r\lor D^\prime$}
%     \BinaryInfC{$(t\simeq s \lor D)[r]\lor D^\prime$}
%     \BinaryInfC{$((C[t]_p\lor D)[r]\lor D^\prime)[t[r]]_{p_1}...[t[r]]_{p_n}$}
%     \AxiomC{$(t\simeq s \lor D)[r]\lor D^\prime$}
%     \BinaryInfC{$((C[t]_p\lor D)[r]\lor D^\prime)[s[r]]_{p_1}...[t[r]]_{p_n}$}
%     \noLine
%     \UnaryInfC{$...$}
%     \noLine
%     \UnaryInfC{$((C[t]_p\lor D)[r]\lor D^\prime)[s[r]]_{p_1}...[t[r]]_{p_n}$}
%     \AxiomC{$(t\simeq s \lor D)[r]\lor D^\prime$}\insertBetweenHyps{\hskip -20pt}
%     \BinaryInfC{$((C[t]_p\lor D)[r]\lor D^\prime)[s[r]]_{p_1}...[s[r]]_{p_n}$}
% \end{prooftree}
% Case 1.2: $t\triangleleft l$ and $p$ has a prefix $q$ where $C|_q=l$:
% \begin{prooftree}
%     \AxiomC{$(C[l[s]_p]_q)[l]$}
%     \AxiomC{$(t\simeq s \lor D)[l]$}
%     \BinaryInfC{$(C[l[t]_p]_q\lor D)[l]$}
%     \AxiomC{$l[t]_p\simeq r\lor D^\prime$}
%     \BinaryInfC{$(C\lor D)[r]\lor D^\prime$}
% \end{prooftree}
% First note that $t\simeq s$ cannot contain $l$. Therefore, we can rewrite $t\simeq s\lor D[l]$ into $t\simeq s\lor D[r]\lor D^\prime$. Then, we perform the following chain of inferences, since $t\succeq s$:
% \begin{prooftree}
%     \AxiomC{$(C[l[s]_p]_q])[l][t]$}
%     \AxiomC{$t\simeq s\lor D[r]\lor D^\prime$}
%     \BinaryInfC{$(C[l[s]_p]_q])[l][s]\lor D[r]\lor D^\prime$}
%     \AxiomC{$(l[t]_p\simeq r\lor D^\prime)[t]$}
%     \AxiomC{$t\simeq s\lor D[r]\lor D^\prime$}
%     \BinaryInfC{$(l[s]_p\simeq r\lor D^\prime)[s]\lor D[r]\lor D^\prime$}
%     \BinaryInfC{$(C[l[s]_p]_q])[r][s]\lor D[r]\lor D^\prime$}
% \end{prooftree}
% Then, since there may be terms $s$ in the conclusion that are terms $t$ in the original conclusion and there may be terms $r$ in the conclusion that are terms $l[s]$ in the original conclusion, we have to repair these by perform \UPar inferences at the end. Note that if $l[s]_p\preceq r$, we can perform a number of \UPar inferences to rewrite the terms $l[s]_p$ in positions that are terms $r$ in the original conclusion and no \UPar inferences are additionally needed with the right premise.

% \noindent
% \textit{Case 2.1}:
% \begin{prooftree}
%     \AxiomC{$C[l[t]_p]$}
%     \AxiomC{$l[s]_p\simeq r\lor D^\prime$}
%     \AxiomC{$t\simeq s\lor D$}
%     \BinaryInfC{$l[t]_p\simeq r\lor D\lor D^\prime$}
%     \BinaryInfC{$C[r]\lor D\lor D^\prime$}
% \end{prooftree}
% We first rewrite every occurrence of $t$ in both $C[l[t]_p]$ and $l[t]_p\simeq r\lor D^\prime$. Note that $t\not\trianglelefteq s$. If $l[s]_p\preceq r$, then we perform a number of \UPar inferences to first rewrite all terms $l[s]_p$ that were originally $l[t]_p$ in the leftmost premise, then perform a number \UPar inferences to rewrite the terms $s$ that should be terms $t$ in the original conclusion. In this case, the new \UPar inferences have rank one less than the original \UPar inference and therefore all multisets are either the same or less in $M(T)$.

% If $l[s]_p\succ r$
% \begin{prooftree}
%     \AxiomC{$(C[l[t]_p])[t]$}
%     \AxiomC{$t\simeq s\lor D$}
%     \BinaryInfC{$(C[l[s]_p])[s]\lor D$}
%     \AxiomC{$(l[s]_p\simeq r\lor D^\prime)[t]$}
%     \AxiomC{$t\simeq s\lor D$}
%     \BinaryInfC{$(l[s]_p\simeq r\lor D^\prime)[s]\lor D$}
%     \BinaryInfC{$(C[r]\lor D^\prime)[r]\lor D$}
% \end{prooftree}
% \textit{Case 2.2}:
% \begin{prooftree}
%     \AxiomC{$C[l]$}
%     \AxiomC{$l\simeq r[s]_p\lor D^\prime$}
%     \AxiomC{$t\simeq s\lor D$}
%     \BinaryInfC{$l\simeq r[t]_p\lor D\lor D^\prime$}
%     \BinaryInfC{$C[r[t]_p]\lor D\lor D^\prime$}
% \end{prooftree}
% Note that $l\succ r[t]_p\succeq r[s]_p$. Therefore, we can perform the rewrite with $l\simeq r[s]_p\lor D^\prime$ first and then rewrite each $r[s]_p$ into $r[t]_p$ by $n$ \UPar inferences. Therefore, we get multisets where $r(I)$ is replaced by $r(I)-1$ with multiplicity $n$.

% \noindent
% \textit{Case 2.3}:
% \begin{prooftree}
%     \AxiomC{$C[l]$}
%     \AxiomC{$l\simeq r\lor D^\prime[s]_p$}
%     \AxiomC{$t\simeq s\lor D$}
%     \BinaryInfC{$l\simeq r\lor D\lor D^\prime[t]_p$}
%     \BinaryInfC{$C[r]\lor D\lor D^\prime[t]_p$}
% \end{prooftree}
% The two inferences can be switched in a straightforward way and each resulting multiset remains the same or has an element which decreased by one.\qed
% \end{proof}


% Yet another alternative proof (with standard non-simultaneous superposition):
% \begin{proof}
% Case 1.1: $p$ is parallel to all positions of $l$ or $l\trianglelefteq t$:
% \begin{prooftree}
%     \AxiomC{$L[s]_p[l]\lor C$}
%     \AxiomC{$t\simeq s \lor D$}
%     \BinaryInfC{$L[t]_p[l]\lor C\lor D$}
%     \AxiomC{$l\simeq r\lor D^\prime$}
%     \BinaryInfC{$L[t]_p[r]\lor C\lor D\lor D^\prime$}
% \end{prooftree}
% The transformed tree is as follows:
% \begin{prooftree}
%     \AxiomC{$L[s]_p[l]\lor C$}
%     \AxiomC{$l\simeq r\lor D^\prime$}
%     \BinaryInfC{$L[s]_p[r]\lor C\lor D^\prime$}
%     \AxiomC{$t\simeq s \lor D$}
%     \BinaryInfC{$L[t]_p[r]\lor C\lor D\lor D^\prime$}
% \end{prooftree}
% Case 1.2: $t\triangleleft l$ and $p$ has a prefix $q$ where $L|_q=l$:
% \begin{prooftree}
%     \AxiomC{$L[l[s]_p]_q[l[t]_p]\lor C$}
%     \AxiomC{$t\simeq s \lor D$}
%     \BinaryInfC{$L[l[t]_p]_q[l[t]_p]\lor C\lor D$}
%     \AxiomC{$l[t]_p\simeq r\lor D^\prime$}
%     \BinaryInfC{$L[r]\lor C\lor D\lor D^\prime$}
% \end{prooftree}
% First note that $t\simeq s$ cannot contain $l$.
% \begin{prooftree}
%     \AxiomC{$(l[t]_p\simeq r\lor D^\prime)[t]$}
%     \AxiomC{$t\simeq s\lor D[r]\lor D^\prime$}
%     \BinaryInfC{$(l[s]_p\simeq r\lor D^\prime)[s]\lor D[r]\lor D^\prime$}
    
% \end{prooftree}
% Case 2.1:
% \begin{prooftree}
%     \AxiomC{$L[l[t]_p]\lor C$}
%     \AxiomC{$l[s]_p\simeq r\lor D^\prime$}
%     \AxiomC{$t\simeq s\lor D$}
%     \BinaryInfC{$l[t]_p\simeq r\lor D\lor D^\prime$}
%     \BinaryInfC{$L[r]\lor C\lor D\lor D^\prime$}
% \end{prooftree}
% Transformed: note that $t\not\trianglelefteq s$
% \begin{prooftree}
%     \AxiomC{$L[l[t]_p][t]\lor C$}
%     \AxiomC{$t\simeq s\lor D$}
%     \BinaryInfC{$L[l[s]_p][s]\lor C\lor D$}
%     \AxiomC{$(l[s]_p\simeq r)[t]\lor D^\prime$}
%     \AxiomC{$t\simeq s\lor D$}
%     \BinaryInfC{$(l[s]_p\simeq r)[s]\lor D^\prime\lor D$}
%     \BinaryInfC{$L[r]\lor C\lor D^\prime\lor D$}
% \end{prooftree}
% Case 2.2:
% \begin{prooftree}
%     \AxiomC{$C[l]$}
%     \AxiomC{$l\simeq r[s]_p\lor D^\prime$}
%     \AxiomC{$t\simeq s\lor D$}
%     \BinaryInfC{$l\simeq r[t]_p\lor D\lor D^\prime$}
%     \BinaryInfC{$C[r[t]_p]\lor D\lor D^\prime$}
% \end{prooftree}
% Transformed:
% \begin{prooftree}
%     \AxiomC{$C[l]$}
%     \AxiomC{$l\simeq r[s]_p\lor D^\prime$}
%     \BinaryInfC{$C[r[s]_p]\lor D^\prime$}
%     \AxiomC{$t\simeq s\lor D$}
%     \dottedLine
%     \BinaryInfC{$C[r[t]_p]\lor D\lor D^\prime$}
% \end{prooftree}
% Case 2.3:
% \begin{prooftree}
%     \AxiomC{$C[l]$}
%     \AxiomC{$l\simeq r\lor D^\prime[s]_p$}
%     \AxiomC{$t\simeq s\lor D$}
%     \BinaryInfC{$l\simeq r\lor D\lor D^\prime[t]_p$}
%     \BinaryInfC{$C[r]\lor D\lor D^\prime[t]_p$}
% \end{prooftree}
% Transformed:
% \begin{prooftree}
%     \AxiomC{$C[l]$}
%     \AxiomC{$l\simeq r\lor D^\prime[s]_p$}
%     \BinaryInfC{$C[r]\lor D^\prime[s]_p$}
%     \AxiomC{$t\simeq s\lor D$}
%     \BinaryInfC{$C[r]\lor D^\prime[t]_p\lor D$}
% \end{prooftree}
% \end{proof}



%%%%%%%%%%%%



\CommentedOut{ we restrict the application of \UPar inferences to only those clauses over which \Ind might be applied, that is to ground clauses only.  We hence  impose the additional restriction on \UPar inferences that \textit{the literal rewritten in the main premise must be ground}; we denote the \SymPar{} calculus variant with such a restriction by \SymPar{}*. Our main result in this section is stated below.

Theorem~\eqref{thm:singleliteral} can be used as follows: given a clause $L\lor C$ with ground literal $L$ that we want to disprove, we perform \SymPar{}* inferences on this clause until $L$ can be proven. Then, we proceed with the rest of the clause.\todo{Explain this better.} 
}

% \begin{lemma}\label{above-position-lemma}
% Given two clauses $L\db{t[r]}\lor C$ and $l\simeq r$ with $l\succ r$, any clause from an $\mtt{Ind}$ inference on term $t[l]$ in literal $L\db{t[l]}$ in clause $L\db{t[l]}\lor C\lor D$ is subsumed by a clause from an $\mathsf{Ind}$ inference on term $t[r]$ in literal $L\db{t[l]}$ in $L\db{t[l]}\lor C$.
% \end{lemma}

% \section{Lifting the calculus}

% Although the \SymPar{} introduced in Section~\ref{sec:Par:LemmaGen} work on general clauses, in the non-ground case and in particular used for auxiliary lemma generation for induction, we have to make some careful considerations additionally, which we discuss in this section.

% \subsection{Rewriting under variable positions and function congruence}

% Full equalitional reasoning includes the reflexivity, commutativity, transitivity and congruence axioms. It is easy to see that \mtt{EqRes} corresponds to reflexivity and commutativity and transitivity is covered by paramodulation, or any special case of it. What about congruence? The congruence axiom for an $n$-ary function $f$ is the following formula:

% $$\forall x_1,...,x_n,y_1,...,y_n.x_1\simeq y_1\land ...\land x_n\simeq y_n\rightarrow f(x_1,...,x_n)\simeq f(y_1,...,y_n)$$

% In \SymPar{} as well as in the \Par{} inference, similarly to the superposition inference in \Sup{}, only non-variable terms are considered from the main premise (c.f. condition (1)). While this is sufficient for first-order completeness, when considering auxiliary lemma generation for induction, we in fact lose lemmas without superpositions at or under variable positions. TBD

% \begin{itemize}
% \item Skipping inductions and \UPar inferences changes a bit since we may have variables and can perform more simplifications.
% \end{itemize}

\CommentedOut{We added options to control the various techniques employed, such as selecting which calculus to use (ADD), and toggling heuristics (ADD).

\todo{in our experiments, we should control and compare \SymPar{}, $\SymPar_G$ and single-literal induction in $\SymPar_G$. The Vampire options should also reflect this}
}
% \section{Erasing equations}

% \begin{definition}
% An equation $l\simeq r$ is called \textit{erasing} if $Var(l)\setminus Var(r)$ is non-empty. 
% \end{definition}

% The following lemma states that no erasing equation can be oriented right-to-left in a simplification ordering.
% \begin{lemma}
% Let $l\simeq r$ be an erasing equation and $\succ$ a simplification ordering. Then, $r\nsucc l$.
% \end{lemma}
% \begin{proof}
% Let $v\in Var(l)\setminus Var(r)$ and assume $r\succ l$. By stability under substitutions, $r\theta\succ l\theta$ for any $\theta$. Let $\theta^\ast=\{v\mapsto r\theta\}\cup\theta$ which is well-defined since $v\notin Var(r)$. Then, $r\theta=r\theta^\ast\succ l\theta^\ast\trianglerighteq r\theta$, contradiction.\qed
% \end{proof}

% The above result means that remodulation possibly "creates" new variables. Since our current induction framework can only deal with ground literals, we need to instantiate them at some point. Let us illustrate this in the following example.
% \begin{example}
% Let us consider a variant of conjecture \eqref{eq:conj1} where we are given an uninterpreted function $g$ with two arguments instead of $f$: 
% \begin{equation*}
% \len(\rev(\append(g(\sigma_0,\sigma_1),\sigma_2))) \not\simeq \suc(\add(\len(\sigma_1),\len(\sigma_2)))
% \end{equation*}
% Also, instead of lemma \eqref{eq:lemma1}, we are supported with the following:
% \begin{equation}%\label{eq:lemma2}
%     \forall x\in\nat,y\in\lst.\ \len(g(x,y))\simeq\suc(\len(y)) 
% \end{equation}
% Similarly as with \eqref{eq:conj1}, we can use \eqref{eq:add2} and \eqref{eq:lemma2} right-to-left but we need to instantiate the newly introduced variable $x$ as $\sigma_0$ to match the other $g$ term:
% \begin{equation*}
% \len(\rev(\append(g(\sigma_0,\sigma_1),\sigma_2))) \not\simeq \add(\len(g(\sigma_0,\sigma_1)),\len(\sigma_2))
% \end{equation*}
% Solving this requires generalizing over $g(\sigma_0,\sigma_1)$.\qed
% \end{example}

% Notice that our choice of instantiating the new variables before inducting on the result are also limited by the redundancy criteria that we used earlier. Namely, in the previous example, instantiating to \textit{anything except for $a$} makes the resulting induction clauses redundant, since either they can be written back with the lemma left-to-right or the induction is done on terms irrelevant for the shape of the induction.

% \section{Optimizing the simplification ordering}


\todo[inline]{UFDTLIA errors:

% 1. (= (tremove (node d (node ld ll lr) r) d) (node ld (tremove (node ld ll lr) ld) r)) should be (= (tremove (node d (node ld ll lr) r) d) (node ld (tremove (node ld ll lr) d) r));

1. filter definition missing from isaplanner/goal75

2. sorted calls rsorted}


\CommentedOut{Our work is  based the observation that finding auxiliary lemmas for inductive problems can be broadly categorized into two groups: lemmas from the first can be essentially generated by applying equality reasoning and generalizations exhaustively, while the second may require synthesis of new terms. Arguably lemmas from the second category can also be generated by e.g. exhaustive bottom-up techniques where the conjuncts of an induction axiom antecedent are generated starting from tautologies. Nevertheless, we hypothesize that the better benefit-to-cost ratio lies in the first, hence we focus on this category.}
\CommentedOut{Therefore we need additional techniques to prove these lemmas and this is where induction comes into the picture: instead of lemmas,  
In a nutshell, our work extends a given set of axioms/formulas with \textit{valid induction axioms} over these lemmas, that is, instances of \textit{valid induction schemas} instantiated from the lemmas, preserving the consistency of the axiom set. }



\CommentedOut{Note that with schema~\eqref{eq:list-schema}, a formula $\forall z.F[z]$ can only be used as an auxiliary  lemma if $F[\nil]$ and $\forall x,y.(F[y]\implies F[\cons(x,y)])$ are both provable; this in turn may however also require auxiliary lemmas, implying that further induction axioms need to be derived. 
}
%e  process of finding induction axioms is perepeated until the axiom set indeed implies the conjecture. Note that the original conjecture itself is also a lemma when it is used to instantiate a schema.

\CommentedOut{Based on the above discussion, it would be reasonable to divide the problem of inductive reasoning into two subtasks, (1) finding lemmas that imply the conjecture given the axioms and (2) finding suitable induction axioms that prove these lemmas. Of course, the two subtasks are often intertwined. For example, lemma generation methods such as theory exploration \cite{HipSpec} enumerate only valid lemmas, without any guarantees that the lemmas are actually useful for proving the conjecture at hand, while goal-oriented techniques often give invalid lemmas: these are either restricted to using generalizations of the conjecture as lemmas \cite{CADE19,CADE21,Aubin,Cruanes17} or derive lemmas based on failed proof attempts \cite{Rippling93} or patterns that often arise in practice \cite{Wand17}.


\begin{remark}
An alternative possibility to treating induction in a special way is adding the induction schemas as higher-order formulas directly to the initial axiom set. Depending on the higher-order instantiation methods used in a particular prover, this might supersede theory exploration or generalization methods.  
\end{remark}
}


% We distinguish special sorts
% called \textit{term algebra sorts}, and function symbols for term algebra sorts called \textit{constructors}.
% We call the ground terms built from
% the constructor symbols of a sort its \textit{term algebra}. 
% We axiomatise term algebras using their \textit{injectivity}, \textit{distinctness},
% \textit{exhaustiveness} and \textit{acyclicity}
% axioms~\cite{POPL17Kovacs}. %In this paper,
% We refer to term algebras
% also as algebraic data types or inductively defined data types.

%\begin{motivatingexample}[continues=motivating-example]


% \paragraph{{\bf Motivating Example -- Continued.}}\label{ex:motivating}
%\begin{example}\label{ex:motivating}
% To motivate the need of auxiliary lemmas during inductive reasoning,  let us consider the functional program and the assertion in Figure~\ref{fig:defs}(a). The functional program \Prog declares the inductively defined datatypes $\nat$ and $\lst$ and defines the recursive functions $\append$, $\rev$ and $\len$ over these datatypes.
% Assertion \Conj states that reversing a non-empty list $\cons(x,y)$ does not change its length, assuming the same property holds for the tail of the list $y$. The semantics of \Prog is captured by the first-order axioms \eqref{eq:nat1}--\eqref{eq:len2} from Figure~\ref{fig:defs}(b); we denote this set of axioms by $\fol(\Prog)$, with all axioms being implicitly universally quantified. Let $\fol(\Conj)$ denote the first-order formalization of \Conj.
% Proving the functional correctness of Figure~\ref{fig:defs}(a) requires proving that $\fol(\Prog)\rightarrow\fol(\Conj)$, which in turn is reduced to proving unsatisfiability of $\fol(\Prog)\wedge \neg\fol(\Conj)$; formulas \eqref{eq:conj-neg-hyp}--\eqref{eq:conj-neg-conc} in Figure~\ref{fig:defs}(b) represent $\cnf(\neg \fol(\Conj))$.  Hence, unsatisfiability of formulas \eqref{eq:nat1}--\eqref{eq:conj-neg-conc} from Figure~\ref{fig:defs}(b) would imply 
% correctness of Figure~\ref{fig:defs}(a). 
% \CommentedOut{\begin{equation}\label{eq:motEx}
%     \forall x,y.\len(\rev(y))\simeq\len(y)\rightarrow \len(\rev(\cons(x,y)))\simeq\len(\cons(x,y))
% \end{equation}
% Saturation-based theorem provers establish validity of formulas by negating, clausifying and refuting them. As such, instead of proving the validity of $\fol(P)\rightarrow\fol(A)$, saturation-based theorem provers check the unsatisfiability of $\fol(P)\land \neg \fol(A)$, which is shown in Figure~\ref{fig:defs}(b).
% }
% Using the following structural induction schema for natural numbers of lists
% \begin{equation}\label{eq:list-schema}
%     \big(F[\nil]\land\forall x,y.(F[y]\rightarrow F[\cons(x,y)])\big)\rightarrow\forall z.F[z]
% \end{equation}
% where $F$ is an arbitrary formula with one free variable, we can instantiate the following induction formula:
% {\small
% \begin{equation}\label{eq:indf1}
%     \begin{pmatrix}
%         \len(\rev(\nil))\simeq\len(\nil)\land\\ \forall y,z.
%         \begin{pmatrix}
%             \len(\rev(z))\simeq\len(z)\rightarrow \\\len(\rev(\cons(y,z)))\simeq\len(\cons(y,z)))
%         \end{pmatrix}
%     \end{pmatrix}\rightarrow \forall x. \len(\rev(x))\simeq\len(x)
% \end{equation}
% }
% Clausifying \eqref{eq:indf1} results in two clauses, introducing two more Skolem constants $\sigma_1$ and $\sigma_2$:
% {\small
% \begin{align}
%     &\len(\rev(\nil))\not\simeq\len(\nil)\lor \len(\rev(\sigma_2))\simeq\len(\sigma_2)\lor\len(\rev(x))\simeq\len(x)\label{eq:indf1.1}\\
%     &\len(\rev(\nil))\not\simeq\len(\nil)\lor \len(\rev(\cons(\sigma_1,\sigma_2)))\not\simeq\len(\cons(\sigma_1,\sigma_2))\nonumber\\
%     &\hspace{22.7em}\lor\len(\rev(x))\simeq\len(x)\label{eq:indf1.2}
% \end{align}
% }
% Our approach for automating inductive reasoning is \textit{goal-oriented}. That is, instead of introducing instances of induction formulas into the search space and -- after proving their antecedents -- letting their conclusions (here $\len(\rev(x))\simeq\len(x)$) interact as free lemmas, we only instantiate these formulas on demand and disallow any inference with them apart from binary resolution with the conclusion literals as resolvents.
% Upon instantiating formula \eqref{eq:indf1}, our intention is to \textit{induct on} clause \eqref{eq:motExNeg} with induction term $\sigma$, replacing the latter with variables in the instantiation. Thus, we resolve clause \eqref{eq:motExNeg} against clauses \eqref{eq:indf1.1} and \eqref{eq:indf1.2}, binding the variable $x$ to $\sigma$, inducting on \eqref{eq:motExNeg} with induction term $\sigma$ to obtain the following clauses:
% {\small
% \begin{align}
%     &\len(\rev(\nil))\not\simeq\len(\nil)\lor \len(\rev(\sigma_2))\simeq\len(\sigma_2)\label{eq:indf1.1.1}\\
%     &\len(\rev(\nil))\not\simeq\len(\nil)\lor \len(\rev(\cons(\sigma_1,\sigma_2)))\not\simeq\len(\cons(\sigma_1,\sigma_2))\label{eq:indf1.2.1}
% \end{align}}
% Using the base case of $\rev$ \eqref{eq:rev1} on the first literals of \eqref{eq:indf1.1.1}--\eqref{eq:indf1.2.1}, and then using equality resolution, we prove the base case of formula \eqref{eq:indf1.1}. What remains is two unit clauses with the step case hypothesis and conclusion:
% \begin{align}
%     &\len(\rev(\sigma_2))\simeq\len(\sigma_2)\label{eq:indfhyp}\\
%     &\len(\rev(\cons(\sigma_1,\sigma_2)))\not\simeq\len(\cons(\sigma_1,\sigma_2))\label{eq:indfconc}
% \end{align}
% Yet, using only the clauses \eqref{eq:nat1}--\eqref{eq:conj-neg-conc} from Figure~\ref{fig:defs}(b), 
% we can only establish satisfiability of \eqref{eq:nat1}--\eqref{eq:conj-neg-conc}, even though Figure~\ref{fig:defs}(a) is correct. However, when using additional axioms over lists in conjunction with \eqref{eq:nat1}--\eqref{eq:conj-neg-conc}, Figure~\ref{fig:defs}(a) can be proved correct. 
% Namely, consider the following valid first-order property: 
% \begin{equation}
%     \forall u,v.\len(\append(v,\cons(u,\nil)))\simeq\suc(\len(v))\label{eq:lemma}\tag{\sf lemma}
% \end{equation}
% capturing the first-order semantics of a program assertion \Lem given by
% \begin{equation*}
%    \textbf{assert }\len(\append(v,\cons(u,\nil)))=\suc(\len(v))
% \end{equation*}
% We write $\fol(\Lem)$ to denote \eqref{eq:lemma}. 
% As already discussed, $\fol(\Prog)\land\neg\fol(\Conj)$ is not unsat and the auxiliary lemma $\fol(\Lem)$ is needed additionally to establish the validity of \Conj.




\CommentedOut{

Consider now the following assertion \Lem:
\begin{equation*}
    \textbf{assert }\len(\append(v,\cons(u,\nil)))=\suc(\len(v))
\end{equation*}
\noindent
Assertion \Lem is stronger than \Conj in that $\fol(\Lem)\rightarrow\fol(\Conj)$ given $\fol(\Prog)$. Equivalently, $\fol(\Prog)\land\fol(\Lem)\rightarrow\fol(\Conj)$ holds and the superposition calculus can establish unsatisfiability of its negation $\fol(\Prog)\land\fol(\Lem)\land\neg\fol(\Conj)$, where $\fol(\Lem)$ is the following formula:
\begin{equation}
    \forall u,v.\len(\append(v,\cons(u,\nil)))\simeq\suc(\len(v))\label{eq:lemma}
\end{equation}
Therefore, formula~\eqref{eq:lemma} is the lemma needed for proving assertion \Conj and adding it to the clause set in Figure~\ref{fig:defs}(b) makes it unsatisfiable. However, adding formula~\eqref{eq:motEx} also makes the clause set unsatisfiable, since it is the exact negation of clauses~\eqref{eq:conj-neg-hyp} and \eqref{eq:conj-neg-conc}, so why do we use formula~\eqref{eq:lemma}?



Let us denote the quantifier-free part of formula~\eqref{eq:lemma} with $F(u,v)$. One explanation for why formula~\eqref{eq:lemma} is a better lemma than formula~\eqref{eq:motEx} is that both $\forall u.F(u,\nil)$ and $\forall u,x,y.(F(u,y)\rightarrow F(u,\cons(x,y)))$ are implied by axioms \eqref{eq:nat1}-\eqref{eq:cnt2.2} and therefore the instance of schema~\eqref{eq:list-schema} instantiated with $\forall u.F(u,v)$ (note the free variable $v$) can be used to refute the clause set. In contrast, it is very hard to find an instance of an induction schema of formula~\eqref{eq:motEx} with the same properties\footnote{In fact, we could not find any such instance.}. A more intuitive reason for this contrast is that formula~\eqref{eq:lemma} does not contain $\rev$, while formula~\eqref{eq:motEx} does, making any reasoning on the latter harder.

In our induction approach, a necessary condition to instantiate an induction schema with a formula is that the formula can be directly used in an inference with the negated conjecture or one of its descendants. This heuristic is reasonable in a refutational setting, where -- unless the axiom set is inconsistent -- the negated conjecture must be involved in any proof. 
}


\CommentedOut{
\paragraph{{\bf Paper Overview.}} We investigate equality reasoning inferences with weaker restrictions than those of ordered superposition calculi for efficiently deriving (negated instances of) auxiliary lemmas such as \eqref{eq:conj-neg-conc3} in Section~\ref{sec:Par:efficiency}. We further make our inferences efficient by integrating them into saturation and restricting them with observations specific to inductive reasoning in Section~\ref{sec:Par:LemmaGen}. As a result, our techniques allow us to establish correctness of Figure~\ref{fig:defs}(a) by outperforming existing approaches in the area (Sec.~\ref{sec:experiments}). 
}
\CommentedOut{
Example~\ref{ex:motivating} demonstrates some of the challenges of inductive lemma generation using paramodulation. In this paper, our goal is to show validity of a conjecture $F$ possibly requiring inductive reasoning given a set of axioms $\mathcal{A}$. Towards this, we try to establish unsatisfiability of the clause set $\mathcal{C}$ (initially $\cnf(\mathcal{A}\cup\{\neg F\})$) by first-order and inductive reasoning. For the latter, we enumerate clause sets $\mathcal{D}$ implied by $\mathcal{C}$ using paramodulation, then extend out axiom set with instantiations of a fixed set of induction schemas based on lemmas that are generalizations of negated clauses in $\mathcal{D}$. We repeat the process on the clause set until we find the refutation and with it the set of induction axioms needed. Towards this goal, the following research questions can be posed:
\begin{enumerate}
    \item How should we extend the superposition calculus so that unordered paramodulation can be used efficiently?
    \item Can we detect when the induction axioms are enough for a refutation? What guarantees that the clauses we infer are useful for induction?
    \item Is it possible to help inductive reasoning with redundancy from the superposition calculus?
    \item What is the limit of this calculus? What kind of lemmas can be generated and what still cannot be?
\end{enumerate}
}


%nd show that our  method outperforms lemma generation based on superposition without affecting the overall performance much for inductive problems.

% Let us consider the following conjecture:
% \begin{equation}\label{eq:conj1}
%     \len(\rev(\append(f(\sigma_1),\sigma_2))) \not\simeq \suc(\add(\len(\sigma_1),\len(\sigma_2)))
% \end{equation}
% We are also given the following function definition axioms:


% \begin{align}
%     \forall y\in\nat.\ \add(\zero,y) &\simeq y\label{eq:add1}\\
%     \forall x,y\in\nat.\ \add(\suc(x),y) &\simeq \suc(\add(x,y))\label{eq:add2}\\
%     \forall y\in\lst.\ \append(\nil,y) &\simeq y\label{eq:app1}\\
%     \forall x\in\nat,y,z\in\lst.\ \append(\cons(x,y),z) &\simeq \cons(x,\append(y,z))\label{eq:app2}\\
%     \rev(\nil) &\simeq \nil\label{eq:rev1}\\
%     \forall x\in\nat, y\in\lst.\ \append(\rev(x),\cons(y,\nil)) &\simeq \rev(\cons(x,y))\label{eq:rev2}\\
%     \len(\nil) &\simeq \zero\label{eq:len1}\\
%     \forall x\in\nat, y\in\lst.\ \len(\cons(x,y)) &\simeq \suc(\len(y))\label{eq:len2}
% \end{align}

% Moreover, the uninterpreted $f$ is of type $\lst\rightarrow\lst$ and for our purposes, it characterized by the following axiom:
% \begin{equation}\label{eq:lemma1}
%     \forall y\in\lst.\ \len(f(y))\simeq\suc(\len(y)) 
% \end{equation}
% That is, our knowledge about $f$ is that it makes the output list one element longer. A conjecture like \eqref{eq:conj1} is usually proven by structural induction, since it involves datatypes and recursive functions. We can notice that it is very hard to prove \eqref{eq:conj1} with $f$, since it makes $\sigma_1$ stuck on the left hand side, and also, the way $\add$ and $\append$ are defined renders any inductions on $\sigma_2$ useless.

% Using axiom \eqref{eq:add2} and then lemma \eqref{eq:lemma1}, both right-to-left, we get the following:
% \begin{equation}\label{eq:conj2}
%     \len(\rev(\append(f(\sigma_1),\sigma_2))) \not\simeq \add(\len(f(\sigma_1)),\len(\sigma_2))
% \end{equation}
% This makes it possible for us to generalize over $f(\sigma_1)$ and get rid $f$ completely. Without getting much into the details, the induction on $f(\sigma_1)$ results in the following two clauses:
% \begin{align}
%     \begin{split}\len(&\rev(\append(\nil,\sigma_2)))\not\simeq \add(\len(\nil),\len(\sigma_2))\ \lor\ \\ &\len(\rev(\append(\sigma_4,\sigma_2))) \simeq \add(\len(\sigma_4),\len(\sigma_2))\label{eq:ind1.1}\end{split}\\
%     \begin{split}\len(&\rev(\append(\nil,\sigma_2)))\not\simeq \add(\len(\nil),\len(\sigma_2))\ \lor\ \\ &\len(\rev(\append(\cons(\sigma_3,\sigma_4),\sigma_2))) \not\simeq \add(\len(\cons(\sigma_3,\sigma_4)),\len(\sigma_2))\label{eq:ind1.2}\end{split}
% \end{align}
% Let us denote $\len(\rev(\append(\nil,\sigma_2)))\not\simeq \add(\len(\nil),\len(\sigma_2))$ with $C$ and first focus on the step case. Using axioms \eqref{eq:app2}, \eqref{eq:rev2} and \eqref{eq:len2}, we simplify the step case conclusion in \eqref{eq:ind1.2} to this point:
% \begin{align*}
%     &C\lor\len(\append(\rev(\append(\sigma_4,\sigma_2)),\cons(\sigma_3,\nil))) \not\simeq \add(\suc(\len(\sigma_4)),\len(\sigma_2))
% \end{align*}
% If we perform one more induction at this point on the step conclusion literal, we either overgeneralize (try to prove something false) or get bigger and bigger terms without progressing anywhere. Our aim instead is to use the induction hypothesis from \eqref{eq:ind1.1}, to have $\rev(\append(\sigma_4,\sigma_2))$ on both sides so we can perform a generalized induction. To achieve this, we first need to rewrite with \eqref{eq:add2} left-to-right:
% \begin{align*}
%     &C\lor\len(\append(\rev(\append(\sigma_4,\sigma_2)),\cons(\sigma_3,\nil))) \not\simeq \suc(\add(\len(\sigma_4),\len(\sigma_2)))
% \end{align*}
% Finally, we can use the induction hypothesis from \eqref{eq:ind1.1}:
% \begin{align*}
%     &C\lor\len(\append(\rev(\append(\sigma_4,\sigma_2)),\cons(\sigma_3,\nil))) \not\simeq \suc(\len(\rev(\append(\sigma_4,\sigma_2))))
% \end{align*}
% Notice that in order to solve this case, we need to use axiom \eqref{eq:add2} but this time, in a left-to-right orientation, as opposed to when we used it to get \eqref{eq:conj2} from \eqref{eq:conj1}. The superposition calculus disallows rewriting with an equation in both orientations and for completeness within pure first-order logic, this is a reasonable restriction. 

% However, as we can see, in the context of inductive theorem proving, this can be a limiting factor even in case of proving very simple theorems. Apart from this particular case, there can be equations like \eqref{eq:add2}, \eqref{eq:app2}, \eqref{eq:rev2} or the induction hypothesis from \eqref{eq:ind1.1} that can be oriented in many ways, depending on the used simplification ordering, the order of these axioms in the input and so on, which would prevent us from finding a proof for seemingly arbitrary reasons.

% In this paper, we propose inference rules that overcome this limitation and develop some redundancy criteria to avoid performing too many inductions.


% \ifbool{shortversion}{
% }{ % long version:
% \todo[inline]{TODO: Make sure the above paragraphs cover the notation used in the paper and nothing more.}
% } % end of longversion


\CommentedOut{A simplified saturation algorithm for a sound inference system $\mathcal{I}$
is given in Algorithm~\ref{alg:saturation}, with a clausified goal $G$ ($\neg G$ is also clausified) and clausified assumptions $A$ as input.}


\CommentedOut{


\begin{algorithm}[t]
\caption{The Saturation Loop.\label{alg:saturation}}
\begin{tabbing}
	{\scriptsize 1}\quad initial set of clauses $S:=A\cup\{\neg B\}$\\ %active:=\emptyset$\\
	{\scriptsize 2}\quad \reserved{\texttt{repeat}}\\
	{\scriptsize 3}\quad\quad Select  clause $G\in S$\\
	{\scriptsize 4}\quad\quad Derive consequences ${C_1,\ldots,C_n}$ of $G$ and formulas from $S$ using rules of $\mathcal{I}$\\
	{\scriptsize 5}\quad\quad $S:=S\cup \{C_1,\ldots,C_n\}$\\
%	{\scriptsize 6}\quad\quad $active := active\cup\{G\}$\\
	{\scriptsize 6}\quad\quad \reserved{\texttt{if}} $\square\in S$ \reserved{\texttt{then}}~ \reserved{\texttt{return}}~ $A\implies B$ is UNSAT\\
	{\scriptsize 8}\quad \reserved{\texttt{return}}~ $A\implies B$ is SAT
\end{tabbing}
\end{algorithm}
}

\CommentedOut{Note that a saturation algorithm proves validity of $B$ by establishing unsatisfiabiliy of $\neg B$; we refer to this proving process as a {\it refutation} of $\lnot B$ from $A$. }


\CommentedOut{For efficiency reasons, modern saturation-based provers extend revise the $\Sup$ calculus with additional simplifying instances of $\Sup$ rules in order to eliminate redundant
clauses from the search space. 
In our work, we use and adjust the recently introduced 
%; \textit{simplification and deletion rules} are used  to remove redundant clauses during saturation. 
%One simplification rule is a special instance of superposition when one of the
%premises of the superposition rules is a unit clause, yielding the so-called 
%\textit{demodulation} rules, that is, \emph{rewriting by a unit equality}.
\textit{encompassment demodulation} inference~\cite{Duarte2022}.
% In particular, we introduce the so-called \textit{non-unit demodulation $(\NUDem)$} simplifying inference rule, implementing  stronger side conditions than~\cite{Duarte2022}:
% \bigskip
}

% \begin{tabular}{c p{.15\linewidth} l}\label{rule:NUDem}
% \multirow{2}{*}{
% \AxiomC{$l\simeq r$}
% \AxiomC{$C[l\theta]$}
% \LeftLabel{$(\NUDem)$}
% \BinaryInfC{$C[r\theta]$}
% \DisplayProof}
% &
% \multirow{2}{*}{where} 
% &
% (1) $l\theta\succ r\theta$,\\
% & & (2) $C[l\theta]$ is not a unit clause.
% \end{tabular}

\CommentedOut{As described in \cite{CADE19}, in this \Ind inference we get intermediate clauses in form of the clausified induction formula, which are then binary resolved with the premise with resolvent $L[t]$.
}
% Clauses resulting from the clausification of an induction axiom $F\rightarrow \forall x.L\db{x}$ are called \textit{induction clauses}; in addition, we refer to $L\db{t}$ as the \textit{conclusion literal} of the induction axiom.

\CommentedOut{
when a sequence of binary resolutions is performed between the induction clauses of $F\rightarrow \forall x.L\db{t}$ and clause $\overline{L}\db{t}\lor C$ such that the conclusion literals are resolved. We say we 
}



% The rule $(\mathsf{Ind})$ covers generalizations over any term but not over term occurrences. For this, in our work~\cite{CICM20} we introduced a new inference rule with the notable difference that the valid induction formula is $F\rightarrow \forall x.L^\prime[x]$ where $L^\prime[x]$ may contain occurrences of $t$ and $L^\prime[t]=L[t]$.



% \section{Deducing lemmas}

% In this section we discuss our problem of lemma generation on a higher level. In theorem proving, it is common that a set of axioms is given alongside the conjecture we want to prove. That is, we want to verify that:
% $$\mathcal{A}\models C$$
% where $\mathcal{A}$ is the set of axioms and $C$ is the conjecture. Especially with inductive reasoning, sometimes it is easier to prove a set of lemmas from the same set of axioms and use them to prove $C$. In that case, we need to verify the following:
% $$\mathcal{A}\models L_1\quad...\quad\mathcal{A}\models L_n\quad\mathcal{A}\cup\{L_1,...,L_n\}\models C$$
% We can reorder the last part to get:
% $$\mathcal{A}\models (L_1\land...\land L_n)\rightarrow C$$
% Further, using contraposition, we get that:
% $$\mathcal{A}\models \neg C\rightarrow \neg(L_1\land...\land L_n)$$
% Since the above three variants are refuted the same way, i.e. the set $\mathcal{A}\cup\{L_1,...,L_n,\neg C\}$ is refuted, this does not help much. For pure universal lemmas and conjectures, we can use the following implication:
% $$(\exists \overline{x}.F[\overline{x}]\rightarrow \exists \overline{x}.G[\overline{x}])\rightarrow \exists \overline{x}.(F[\overline{x}]\rightarrow G[\overline{x}])$$
% This means that if a universal conjecture can be proven using universal lemmas, then the negation of these lemmas can be deduced from the negated conjecture containing the same Skolem constants.


\CommentedOut{
}


\CommentedOut{
\begin{remark}
\todo{Consider removing this.}
We note a few nice properties of Restriction II. First, it allows further rewritings with the same top-level term. For example, after rewriting $s[l]$ in Figure~\ref{fig:parallelPar}, we necessarily have $s[l]\succ s[r]$;  $s[r]$ thus can be further rewritten. Second, our restriction generalizes to multiple parallel positions across a clause, with the only overhead of storing one extra term per clause. Third, our restriction is not affected by the % it is very easy to maintain, and it is invariant to the exact 
order of literals stored in a clause.
While our restriction still allows equal terms to be rewritten in any order, our experiments show that such situations do not pose a bottleneck in practice. % and imposing further restrictions would make the present discussion less clear.
\end{remark}
}

% For example, the efficiency of the \Sup calculus relies on avoiding either $\Par_c$ or $\Par_d$ in (a) by only superposing the maximal term in the maximal literal w.r.t. $\succ$ (c.f. condition (3) for \mtt{Sup} in Figure~\ref{fig:sup}). Note, however, that avoiding duplicates in case (b) is not addressed by the \Sup calculus, and although it is possible, the additional book-keeping required makes the present discussion less clear, so we also leave it as future work.

% In superposition-based theorem provers, redundancy elimination handles the duplicates of (b), but doing the same for (a) as well can hinder the saturation process significantly.
% % To overcome this burden within applications of $\Par$ while retaining its deriving power, we get inspiration from the restrictions of \Sup for solving (a) as follows. Let us consider downward paramodulations for now on a clause and take the set $S$ of its top-level terms.
% Instead of only rewriting $t=\max_\succ(S)$ as in \Sup, in each iteration, we consider two ``branches'', one where $t$ is rewritten, and one where it is not. Then, we repeat the process with $S\setminus t$ recursively in both branches, in the rewritten branch adding also any new top-level terms  smaller than $t$ to $S$ that are added by the rewrite. It is easy to see that this process generates all possible results of parallel \Par inferences.


% \complthm*
% \begin{proof}
% The ground case is solved by Lemma~\ref{thm:complthm-ground}. For the non-ground case, we additionally have to consider the case that a derivation $\Lambda$ cannot be transformed into a new derivation $\Pi$ because in $\Pi$, one of the terms to be paramodulated would be under a variable position. For example, consider case {\bf (I.1.a)} in the non-ground case, where $\theta=\mgu(w,w^\prime)$ and $\mu=\mgu(l,l^\prime\theta)$ and $l^\prime$ is $x\theta|_p$ for some variable in $C\an{s[l^\prime]]}\an{t[w^\prime]}$
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[l^\prime]]}\an{t[w^\prime]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w\lor D^\prime$}
%     \BinaryInfC{$(C\an{s[l^\prime]}\an{t[u]}\lor D^\prime)\theta\uparrow t[w^\prime]\theta$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l\simeq r \lor D$}
%     \BinaryInfC{$(C\an{s[r]}\an{t[u]}\lor D\lor D^\prime)\theta\mu\downarrow s[l^\prime]\theta\mu$}
%     \DisplayProof
% \end{center} 
% By assumption, $w$ must contain (possibly more than one) non-variable term $l_1$,...,$l_n$ that unifies with $l$. For simplicity, we only deal with the instance $(u\simeq w\lor D^\prime)\theta$ that is used in the above derivation. This will make the argument more clear, yet, all inferences shown can still be performed in on the original clauses as we perform rewrites above variable positions.

% There are two cases, either  $t[w^\prime]$ contains non-variable terms that instantiate to $l\theta$ or not. In the first case, we rewrite $l\theta$ with $(l\simeq r\lor D)\theta$ shown below:
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$(u\simeq w[l]...[l]\lor D^\prime)\theta$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$(l\simeq r \lor D)\theta$}
%     \BinaryInfC{$(u\simeq w[r][l]...[l]\lor D\lor D^\prime)\theta\downarrow w[l]...[l]\theta$}
%     \UnaryInfC{$\ddots$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$(l\simeq r \lor D)\theta$}
%     \BinaryInfC{$(u\simeq w[r]...[r]\lor D\lor D^\prime)\theta\downarrow w[r]...[r][l]\theta$}
%     \DisplayProof
% \end{center}
% A similar rewrite chain must be performed on $(C\an{s[l^\prime]}\an{t[w^\prime]})\theta$ in which the non-variable terms that instantiate to $l\theta$ are rewritten into $r\theta$ in $w^\prime\theta$, otherwise $w^\prime\theta$ does not unify with $w[r]...[r]\theta$:
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$(C\an{s[l^\prime]}\an{t[w^\prime[l]...[l]]})\theta$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$(l\simeq r \lor D)\theta$}
%     \BinaryInfC{$(C\an{s[l^\prime]}\an{t[w^\prime[l]...[l]]}\lor D)\theta\downarrow t[w^\prime[l]...[l]]\theta$}
%     \UnaryInfC{$\ddots$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$(l\simeq r \lor D)\theta$}
%     \BinaryInfC{$(C\an{s[l^\prime]}\an{t[w^\prime[r]...[r]]}\lor D)\theta\downarrow t[w^\prime[r]...[r][l]]\theta$}
%     \DisplayProof
% \end{center}
% Finally, we put the two derivations together, to get the following:
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[l^\prime]}\an{t[w^\prime[r]...[r]]}\lor D\downarrow t[w^\prime[r]...[r][l]]$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w[r]...[r]\lor D\lor D^\prime\downarrow w[r]...[r][l]$}
%     \BinaryInfC{$C\an{s[r]}\an{t[u]}\lor D\lor D^\prime\uparrow t[w]$}
%     \DisplayProof
% \end{center}
% If the final clause is the same, we get $T(\Lambda)\ggg T(\Pi)$ and we are done. Otherwise, it is so because some variables have been instantiated with $r$s instead of $l$s in the final clause. TBD.
% \end{proof}


% Counterexample for lifting:
% \begin{itemize}
%     \item non-ground \Par derivation that needs to be transformed:
%     \begin{prooftree}
%     \AxiomC{$g(f(x),x)\simeq x$}
%     \AxiomC{$c\simeq f(l)$}
%     \LeftLabel{$(\Par (upward))$}
%     \BinaryInfC{$g(c,l)\simeq l$}
%     \AxiomC{$l\simeq r$}
%     \RightLabel{$(\Par (downward))$}
%     \BinaryInfC{$g(c,r)\simeq l$}
%     \end{prooftree}
%     \item ground version in \SymPar:
%     \begin{prooftree}
%     \AxiomC{$g(f(l),l)\simeq l$}
%     \AxiomC{$l\simeq r$}
%     \LeftLabel{$(\DPar)$}
%     \BinaryInfC{$g(f(l),r)\simeq l\downarrow g(f(l),l)$}
%     \AxiomC{$c\simeq f(l)$}
%     \RightLabel{$(\UPar)$}
%     \BinaryInfC{$g(c,r)\simeq l\uparrow g(f(l),r)$}
%     \end{prooftree}
%     \item non-ground version in \SymPar:
%     \begin{prooftree}
%     \AxiomC{$g(f(x),x)\simeq x$}
%     \AxiomC{$c\simeq f(l)$}
%     \AxiomC{$l\simeq r$}
%     \RightLabel{$(\DPar)$}
%     \BinaryInfC{$c\simeq f(r)\downarrow f(l)$}
%     \LeftLabel{$(\UPar)$}
%     \BinaryInfC{$g(c,r)\simeq r\uparrow g(f(r),r)$}
%     \end{prooftree}
%     At this point, the equality side $r$ should be rewritten back to $l$ but it cannot be done because $r$ is smaller than the current annotation $f(r)$.
% \end{itemize}
% \noindent\rule{\textwidth}{1pt}

% \begin{example}
%     $$\{a^\prime\not\simeq t, \quad a\simeq a^\prime\lor b^\prime\not\simeq t^\prime,\quad b\simeq b^\prime\}$$
%     $$a\succ a^\prime \succ b\succ b^\prime$$
%     Let's say we want to reach $a\not\simeq t\lor b\not\simeq t^\prime$ to induct on it. In \SymPar{}:
%     \begin{enumerate}
%         \item \UPar with $a\simeq a^\prime\lor b^\prime\not\simeq t^\prime$ and $b\simeq b^\prime$ to obtain $a\simeq a^\prime\lor b\not\simeq t^\prime\uparrow b^\prime$
%         \item \UPar with $a^\prime\not\simeq t$ and $a\simeq a^\prime\lor b\not\simeq t^\prime$ to obtain $a\not\simeq t\lor b\not\simeq t^\prime\uparrow a^\prime$ and condition $a^\prime\succeq b^\prime$ is satisfied
%     \end{enumerate}
%     This cannot be done the other way around since:
%     \begin{enumerate}
%         \item \UPar with $a^\prime\not\simeq t$ and $a\simeq a^\prime\lor b^\prime\not\simeq t^\prime$ to obtain $a\not\simeq t\lor b^\prime\not\simeq t^\prime\uparrow a^\prime$
%         \item \UPar with $a\not\simeq t\lor b^\prime\not\simeq t^\prime\uparrow a^\prime$ and $b\simeq b^\prime$ does not work since $b^\prime\not\succeq a^\prime$
%     \end{enumerate}
%     So we cannot select a "goal" to use \UPar on since both $a^\prime\not\simeq t$ and $a\simeq a^\prime\lor b^\prime\not\simeq t^\prime$ have to be upward paramodulated.
    
%     But, if we use single-literal induction and \SymPar{}*, we can select $a^\prime\not\simeq t$ as goal and do as follows
%     \begin{enumerate}
%         \item \UPar with $a^\prime\not\simeq t$ and $a\simeq a^\prime\lor b^\prime\not\simeq t^\prime$ to obtain $a\not\simeq t\lor b^\prime\not\simeq t^\prime\uparrow a^\prime$
%         \item Induct on $a\not\simeq t$ in $a\not\simeq t\lor b^\prime\not\simeq t^\prime\uparrow a^\prime$ which results eventually in $b^\prime\not\simeq t^\prime$, without the $\updownarrow$ state which is reset during induction
%         \item \UPar with $b^\prime\not\simeq t^\prime$ and $b\simeq b^\prime$ to get $b\not\simeq t^\prime$
%         \item induct on $b\not\simeq t^\prime$
%     \end{enumerate}
% \qed
% \end{example}







% \subsection{Derivability in \SymParG{}}

% In this section, we present the proof of Theorem~\ref{thm:singleliteral}. As in the previous section, we first prove the ground case, and for that, we display the ground rules for \SymParG{} below.

% \begin{mdframed}[frametitle={\colorbox{white}{\space  \SymParG{} Inferences (ground)\space}},
%     innertopmargin=5pt,
%     innerbottommargin=15pt,
%     innerleftmargin=0pt,
%     innerrightmargin=0pt,
%     frametitleaboveskip=-\ht\strutbox,
%     frametitlealignment=\center]

% \begin{tabular}{p{.52\linewidth} p{.12\linewidth} l}
% \multirow{4}{*}{
% \AxiomC{$s[l]\bowtie s^\prime\lor C\downarrow t$}
% \AxiomC{$l\simeq r\lor D\downarrow t^\prime$}
% \LeftLabel{(\DPar)}
% \BinaryInfC{$s[l]\bowtie s^\prime\lor C\lor D\downarrow s[l]$}
% \DisplayProof}
% &
% \multirow{4}{*}{where}
% & (1) $t^\prime\succeq l \succ r$,\\
% & & (2) $t\succeq s[l]$,\\
% & & (3) $s[l]\succ s^\prime$ or\\
% & & \hspace{1.6em}$s[l]\bowtie s^\prime\lor C\downarrow t\in\mathcal{C}_G$.\\
% \\
% \multirow{4}{*}{
% \AxiomC{$C\an{s[r]}\updownarrow t$}
% \AxiomC{$l\simeq r\lor D\updownarrow t^\prime$}
% \LeftLabel{(\UPar)}
% \BinaryInfC{$C\an{s[l]}\lor D\uparrow s[r]$}
% \DisplayProof}
% &
% \multirow{4}{*}{where}
% & (1) $l\succeq r$,\\
% & & (2) $\updownarrow t^\prime=\ \downarrow t^\prime$ or $s[r]\succeq t^\prime$,\\
% & & (3) $\updownarrow t=\ \downarrow t$ or $s[r]\succeq t$,\\
% & & (4) $C\an{s[r]}\updownarrow t\in\mathcal{C}_G$.
% \end{tabular}
% \end{mdframed}

% \begin{definition}[Number of \UPar inferences]
% For a paramodulation derivation $\Lambda=\mathcal{C}\vdash D\updownarrow t$, we define $n(\Lambda)$ as the number of \UPar inferences in the derivation.
% \end{definition}
% We make use of the following consequence of Lemma~\ref{thm:complthm-ground} which can be easily verified based on the proof of Lemma~\ref{thm:complthm-ground}.
% \begin{lemma}\label{n-t-lemma}
% For any \ParC{} derivation $\Lambda=\mathcal{C}\vdash D\updownarrow s$, there is a \SymPar{} derivation $\Pi=\mathcal{C}\vdash D\updownarrow t$, such that $n(\Lambda)\geq n(\Pi)$ and $T(\Lambda)\gggeq T(\Pi)$.
% \end{lemma}

% \begin{lemma}
%     Given a ground \ParC{} derivation resulting in $L^\prime \lor D$ from main premise $L\lor C$ and side premises $\mathcal{C}$ such that the derivation rewrites $L$ into $L^\prime$, there is a ground \SymParG{} derivation resulting $L^\prime \lor D^\prime$ from main premise $L\lor C$ and side premises $\mathcal{C}$ that only rewrites $L$ and a \ParC{} derivation resulting in $D$ from $D^\prime$ and $\mathcal{C}$.
% \end{lemma}
% \begin{proof}
% \noindent\rule{\textwidth}{.2pt}
% \textbf{(I)} The inference is a \UPar inference.\\
% \noindent\rule{\textwidth}{.2pt}
% \textbf{(I.a)} $t^\prime=r[w]$ and $s[r]=s[r[u]]$
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[r[u]]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l\simeq r[w]\lor D$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w \lor D^\prime$}
%     \BinaryInfC{$l\simeq r[u]\lor D\lor D^\prime\uparrow r[w]$}
%     \BinaryInfC{$C\an{s[l]}\lor D\lor D^\prime\uparrow s[r[u]]$}
%     \DisplayProof
% \end{center}
% The new derivation $\Sigma$ contains instead the following inferences:
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[r[u]]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w \lor D^\prime$}
%     \BinaryInfC{$C\an{s[r[w]]}\lor D^\prime\downarrow s[r[u]]$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l\simeq r[w]\lor D$}
%     \BinaryInfC{$C\an{s[l]}\lor D\lor D^\prime\uparrow s[r[w]]$}
%     \DisplayProof
% \end{center}
% $n(\Lambda)\geq n(\Pi)>n(\Sigma)$ yields the claim.\\
% \rule{\textwidth}{.2pt}
% \textbf{(I.b)} $t^\prime=l[w]$ and by assumption $s[r]\succeq l[w]$
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[r]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l[w]\simeq r\lor D$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w \lor D^\prime$}
%     \BinaryInfC{$l[u]\simeq r\lor D\lor D^\prime\uparrow l[w]$}
%     \BinaryInfC{$C\an{s[l[u]]}\lor D\lor D^\prime\uparrow s[r]$}
%     \DisplayProof
% \end{center}
% If $l[w]\succ r$, the new derivation $\Sigma$ contains the following inferences:
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[r]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l[w]\simeq r\lor D$}
%     \BinaryInfC{$C\an{s[l[w]]}\lor D\uparrow s[r]$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w\lor D^\prime$}
%     \BinaryInfC{$C\an{s[l[u]]}\lor D\lor D^\prime\uparrow s[l[w]]$}
%     \DisplayProof
% \end{center}
% Either $n(\Lambda)>n(\Pi)=n(\Sigma)$ or $n(T)=n(T^\ast)=n(T^\prime)$ and $s[l[w]]\succ s[r]$ yields $T(\Lambda)\geq T(\Pi)>T(\Sigma)$. Otherwise:
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[r]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l[w]\simeq r\lor D^\prime$}
%     \BinaryInfC{$C\an{s[l[w]]}\lor D^\prime\downarrow s[r]$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w\lor D$}
%     \BinaryInfC{$C\an{s[l[u]]}\lor D\lor D^\prime\uparrow s[l[w]]$}
%     \DisplayProof
% \end{center}
% $n(\Lambda)\ge n(\Pi)>n(\Sigma)$ yields the claim.\\
% \rule{\textwidth}{.2pt}
% \textbf{(I.c)} $t^\prime=t^\prime[w]$ for some top-level term other than $l$ or $r$.
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[r]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l\simeq r\lor D\an{t^\prime[w]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w \lor D^\prime$}
%     \BinaryInfC{$l\simeq r\lor D\an{t^\prime[u]}\lor D^\prime\uparrow t^\prime[w]$}
%     \BinaryInfC{$C\an{s[l]}\lor D\lor D^\prime\an{t^\prime[u]}\uparrow s[r]$}
%     \DisplayProof
% \end{center}
% By condition (2) of \UPar, $s[r]\succeq t^\prime[w]$. We find the next point in the derivation tree where $t^\prime[u]$ would be used, but we have $t^\prime[w]$ instead.

% \noindent
% (1) It is not used, i.e. the clause at the root of the original derivation tree is $C\an{t^\prime[u]}$. Show that the clause with $t^\prime[w]$ is also unsatisfiable and smaller.

% \noindent
% (2) It is inducted upon, i.e. there is an inference:
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$L\an{t^\prime[u]}\lor C$}
%     \UnaryInfC{$\cnf(\neg F)\lor C$}
%     \DisplayProof
% \end{center}

% \noindent
% (3) It is rewritten, i.e. there is an inference
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{t^\prime[u][l]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l\simeq r\lor D$}
%     \BinaryInfC{$C\an{t^\prime[u][l]}\lor D\downarrow t^\prime[u][l]$}
%     \DisplayProof
% \end{center}
% \noindent\rule{\textwidth}{.2pt}
% \textbf{(I.d)} $l\succ r[u]$ and the upper inference is a \DPar inference on a non-goal clause.
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[r[w]]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l\simeq r[u]\lor D$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w \lor D^\prime$}
%     \BinaryInfC{$l\simeq r[w]\lor D\lor D^\prime\downarrow r[u]$}
%     \BinaryInfC{$C\an{s[l]}\lor D\lor D^\prime\uparrow s[r[w]]$}
%     \DisplayProof
% \end{center}
% The new derivation $\Sigma$ is the following:
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[r[w]]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w \lor D^\prime$}
%     \BinaryInfC{$C\an{s[r[u]]}\lor D^\prime\uparrow s[r[w]]$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l\simeq r[u]\lor D$}
%     \BinaryInfC{$C\an{s[l]}\lor D\lor D^\prime\uparrow s[r[u]]$}
%     \DisplayProof
% \end{center}
% {\color{red}{}Here $n(\Pi)<n(\Sigma)$ (but the other measure decreases).}\\
% \noindent\rule{\textwidth}{.2pt}
% \textbf{(I.e)} $t\succ t^\prime[u]$
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[r]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l\simeq r\lor t\bowtie t^\prime[u]\lor D$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w \lor D^\prime$}
%     \BinaryInfC{$l\simeq r\lor t\bowtie t^\prime[w]\lor D\lor D^\prime\downarrow t^\prime[u]$}
%     \BinaryInfC{$C\an{s[l]}\lor t\bowtie t^\prime[w]\lor D\lor D^\prime\uparrow s[r]$}
%     \DisplayProof
% \end{center}
%  This should be doable after the next induction. TBD.\\
% \noindent\rule{\textwidth}{.2pt}
% \textbf{(II)} The inference is a \DPar inference.\\
% \noindent\rule{\textwidth}{.2pt}
% \textbf{(II.a)} $l\succ r[u]$
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[l]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l\simeq r[u]\lor D$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w \lor D^\prime$}
%     \BinaryInfC{$l\simeq r[w]\lor D\lor D^\prime\downarrow r[u]$}
%     \BinaryInfC{$C\an{s[r[w]]}\lor D\lor D^\prime\downarrow s[l]$}
%     \DisplayProof
% \end{center}
% This yields a contradiction, as $t^\prime=r[u]\succ l\succ r[u]$, therefore this case is not possible.\\
% \rule{\textwidth}{.2pt}
% \textbf{(II.b)} $t\succ t^\prime=t^\prime[u]$
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[l]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l\simeq r\lor t\bowtie t^\prime[u]\lor D$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w \lor D$}
%     \BinaryInfC{$l\simeq r\lor t\bowtie t^\prime[w]\lor D\lor D^\prime\downarrow t^\prime[u]$}
%     \BinaryInfC{$C\an{s[r]}\lor t\bowtie t^\prime[w]\lor D\lor D^\prime\downarrow s[l]$}
%     \DisplayProof
% \end{center}
% By assumption, $t^\prime[u]\succeq l$. This should be doable after the next induction similarly to (c).\\
% \rule{\textwidth}{.2pt}
% \textbf{(II.c)} By assumption, $l\succ r[u]$
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[r[w]]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l\simeq r[u]\lor D$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w \lor D^\prime$}
%     \BinaryInfC{$l\simeq r[w]\lor D\lor D^\prime\downarrow r[u]$}
%     \BinaryInfC{$C\an{s[l]}\lor D\lor D^\prime\uparrow s[r[w]]$}
%     \DisplayProof
% \end{center}
% The transformed tree is as follows:
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[r[w]]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w \lor D$}
%     \BinaryInfC{$C\an{s[r[u]]}\lor D\uparrow s[r[w]]$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l\simeq r[u]\lor D^\prime$}
%     \BinaryInfC{$C\an{s[l]}\lor D\lor D^\prime\uparrow s[r[u]]$}
%     \DisplayProof
% \end{center}
% \rule{\textwidth}{.2pt}
% \end{proof}

% \singleliterallemma*
% \begin{proof}
%     We show the proof in the ground case. The lifting to non-ground clauses is very similar to that of Theorem~\ref{thm:completeness}. Let us assume that we are given a ground refutation using \ParC{}+\IndG from a ground clause set $\mathcal{C}$. We induct on the number of \IndG inferences used. If there are no \IndG inferences in the derivation, then the initial clause set must be already first-order unsatisfiable. Otherwise, first, let us use Lemma~\ref{thm:complthm-ground} to convert each subderivation between \IndG inferences to \SymPar{} derivations.

%     We argue as follows: let us take any subderivation with an ending in an \IndG inference. By definition of goal clauses, going back from the end of the derivation along main premises, we reach a goal clause $D$. In $D$, either there is some literal that -- after possibly rewriting it -- is inducted upon or otherwise there is a literal that is introduced by a paramodulation that will be inducted upon.

%     In the first case, let this $L$ be the literal in $D$ and $L^\prime$ the literal that is finally inducted upon. We can trace the paramodulations producing $L^\prime$ from $L$ in the tree and move them up in order to produce $L^\prime$ directly from $D$. This results in a clause $D^\prime$ that contains $L^\prime$, which can be used in an \IndG inference. If there are any non-\SymParG{} inferences in this derivation resulting in $D^\prime$, it is so because either a \UPar inference is used on a non-goal side premise or a \DPar inference is used on the smaller side of an equality in a non-goal side premise.
% \end{proof}

% \begin{lemma}
%     Given a set of ground clauses $\mathcal{C}$ with a non-empty set of goal clauses. If $\mathcal{C}\vdash_{\ParC{}+\IndG} D\updownarrow s$, then $\mathcal{C}\vdash_{\SymParG{}+\IndG} D\updownarrow t$.
% \end{lemma}
% \begin{proof}
% By induction on the cartesian product $(n(\Lambda),T(\Lambda))$ using the \ParC{} derivation $\Lambda$ with the lexicographic order $(>,\ggg)_{lex}$.

% Given a \ParC{} derivation $\Lambda=\mathcal{C}\vdash_{\ParC{}+\IndG} D\updownarrow s$, we assume the product is minimal w.r.t. the lexicographic product. First, we convert the derivation to a \SymPar{} derivation $\Pi$. By Lemma~\ref{n-t-lemma}, we get $n(\Lambda)\geq n(\Pi)$ and $T(\Lambda)\gggeq T(\Pi)$. Moreover, the subgraph of nodes stemming from \UPar nodes in $T(\Pi)$ is a tree. If $\Pi$ is also a \SymParG{} derivation, we are done. \Blue{Otherwise, there is an inference in $\Pi$ whose main premise is a goal clause and its side premise is the conclusion of a \UPar inference.} Assume $l\succ r$ and $u\succ w$. We transform $\Pi$ into a derivation $\Sigma$ s.t. $n(\Pi)>n(\Sigma)$ or $n(\Pi)=n(\Sigma)$ and $T(\Pi)\ggg T(\Sigma)$.\medskip

% \noindent\rule{\textwidth}{.2pt}
% \textbf{(I)} The inference is a \UPar inference.\\
% \noindent\rule{\textwidth}{.2pt}
% \textbf{(I.a)} $t^\prime=r[w]$ and $s[r]=s[r[u]]$
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[r[u]]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l\simeq r[w]\lor D$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w \lor D^\prime$}
%     \BinaryInfC{$l\simeq r[u]\lor D\lor D^\prime\uparrow r[w]$}
%     \BinaryInfC{$C\an{s[l]}\lor D\lor D^\prime\uparrow s[r[u]]$}
%     \DisplayProof
% \end{center}
% The new derivation $\Sigma$ contains instead the following inferences:
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[r[u]]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w \lor D^\prime$}
%     \BinaryInfC{$C\an{s[r[w]]}\lor D^\prime\downarrow s[r[u]]$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l\simeq r[w]\lor D$}
%     \BinaryInfC{$C\an{s[l]}\lor D\lor D^\prime\uparrow s[r[w]]$}
%     \DisplayProof
% \end{center}
% $n(\Lambda)\geq n(\Pi)>n(\Sigma)$ yields the claim.\\
% \rule{\textwidth}{.2pt}
% \textbf{(I.b)} $t^\prime=l[w]$ and by assumption $s[r]\succeq l[w]$
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[r]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l[w]\simeq r\lor D$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w \lor D^\prime$}
%     \BinaryInfC{$l[u]\simeq r\lor D\lor D^\prime\uparrow l[w]$}
%     \BinaryInfC{$C\an{s[l[u]]}\lor D\lor D^\prime\uparrow s[r]$}
%     \DisplayProof
% \end{center}
% If $l[w]\succ r$, the new derivation $\Sigma$ contains the following inferences:
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[r]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l[w]\simeq r\lor D$}
%     \BinaryInfC{$C\an{s[l[w]]}\lor D\uparrow s[r]$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w\lor D^\prime$}
%     \BinaryInfC{$C\an{s[l[u]]}\lor D\lor D^\prime\uparrow s[l[w]]$}
%     \DisplayProof
% \end{center}
% Either $n(\Lambda)>n(\Pi)=n(\Sigma)$ or $n(T)=n(T^\ast)=n(T^\prime)$ and $s[l[w]]\succ s[r]$ yields $T(\Lambda)\geq T(\Pi)>T(\Sigma)$. Otherwise:
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[r]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l[w]\simeq r\lor D^\prime$}
%     \BinaryInfC{$C\an{s[l[w]]}\lor D^\prime\downarrow s[r]$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w\lor D$}
%     \BinaryInfC{$C\an{s[l[u]]}\lor D\lor D^\prime\uparrow s[l[w]]$}
%     \DisplayProof
% \end{center}
% $n(\Lambda)\ge n(\Pi)>n(\Sigma)$ yields the claim.\\
% \rule{\textwidth}{.2pt}
% \textbf{(I.c)} $t^\prime=t^\prime[w]$ for some top-level term other than $l$ or $r$.
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[r]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l\simeq r\lor D\an{t^\prime[w]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w \lor D^\prime$}
%     \BinaryInfC{$l\simeq r\lor D\an{t^\prime[u]}\lor D^\prime\uparrow t^\prime[w]$}
%     \BinaryInfC{$C\an{s[l]}\lor D\lor D^\prime\an{t^\prime[u]}\uparrow s[r]$}
%     \DisplayProof
% \end{center}
% By condition (2) of \UPar, $s[r]\succeq t^\prime[w]$. We find the next point in the derivation tree where $t^\prime[u]$ would be used, but we have $t^\prime[w]$ instead.

% \noindent
% (1) It is not used, i.e. the clause at the root of the original derivation tree is $C\an{t^\prime[u]}$. Show that the clause with $t^\prime[w]$ is also unsatisfiable and smaller.

% \noindent
% (2) It is inducted upon, i.e. there is an inference:
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$L\an{t^\prime[u]}\lor C$}
%     \UnaryInfC{$\cnf(\neg F)\lor C$}
%     \DisplayProof
% \end{center}

% \noindent
% (3) It is rewritten, i.e. there is an inference
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{t^\prime[u][l]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l\simeq r\lor D$}
%     \BinaryInfC{$C\an{t^\prime[u][l]}\lor D\downarrow t^\prime[u][l]$}
%     \DisplayProof
% \end{center}
% \noindent\rule{\textwidth}{.2pt}
% \textbf{(I.d)} $l\succ r[u]$ and the upper inference is a \DPar inference on a non-goal clause.
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[r[w]]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l\simeq r[u]\lor D$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w \lor D^\prime$}
%     \BinaryInfC{$l\simeq r[w]\lor D\lor D^\prime\downarrow r[u]$}
%     \BinaryInfC{$C\an{s[l]}\lor D\lor D^\prime\uparrow s[r[w]]$}
%     \DisplayProof
% \end{center}
% The new derivation $\Sigma$ is the following:
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[r[w]]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w \lor D^\prime$}
%     \BinaryInfC{$C\an{s[r[u]]}\lor D^\prime\uparrow s[r[w]]$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l\simeq r[u]\lor D$}
%     \BinaryInfC{$C\an{s[l]}\lor D\lor D^\prime\uparrow s[r[u]]$}
%     \DisplayProof
% \end{center}
% {\color{red}{}Here $n(\Pi)<n(\Sigma)$ (but the other measure decreases).}\\
% \noindent\rule{\textwidth}{.2pt}
% \textbf{(I.e)} $t\succ t^\prime[u]$
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[r]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l\simeq r\lor t\bowtie t^\prime[u]\lor D$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w \lor D^\prime$}
%     \BinaryInfC{$l\simeq r\lor t\bowtie t^\prime[w]\lor D\lor D^\prime\downarrow t^\prime[u]$}
%     \BinaryInfC{$C\an{s[l]}\lor t\bowtie t^\prime[w]\lor D\lor D^\prime\uparrow s[r]$}
%     \DisplayProof
% \end{center}
%  This should be doable after the next induction. TBD.\\
% \noindent\rule{\textwidth}{.2pt}
% \textbf{(II)} The inference is a \DPar inference.\\
% \noindent\rule{\textwidth}{.2pt}
% \textbf{(II.a)} $l\succ r[u]$
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[l]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l\simeq r[u]\lor D$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w \lor D^\prime$}
%     \BinaryInfC{$l\simeq r[w]\lor D\lor D^\prime\downarrow r[u]$}
%     \BinaryInfC{$C\an{s[r[w]]}\lor D\lor D^\prime\downarrow s[l]$}
%     \DisplayProof
% \end{center}
% This yields a contradiction, as $t^\prime=r[u]\succ l\succ r[u]$, therefore this case is not possible.\\
% \rule{\textwidth}{.2pt}
% \textbf{(II.b)} $t\succ t^\prime=t^\prime[u]$
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[l]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l\simeq r\lor t\bowtie t^\prime[u]\lor D$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w \lor D$}
%     \BinaryInfC{$l\simeq r\lor t\bowtie t^\prime[w]\lor D\lor D^\prime\downarrow t^\prime[u]$}
%     \BinaryInfC{$C\an{s[r]}\lor t\bowtie t^\prime[w]\lor D\lor D^\prime\downarrow s[l]$}
%     \DisplayProof
% \end{center}
% By assumption, $t^\prime[u]\succeq l$. This should be doable after the next induction similarly to (c).\\
% \rule{\textwidth}{.2pt}
% \textbf{(II.c)} By assumption, $l\succ r[u]$
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[r[w]]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l\simeq r[u]\lor D$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w \lor D^\prime$}
%     \BinaryInfC{$l\simeq r[w]\lor D\lor D^\prime\downarrow r[u]$}
%     \BinaryInfC{$C\an{s[l]}\lor D\lor D^\prime\uparrow s[r[w]]$}
%     \DisplayProof
% \end{center}
% The transformed tree is as follows:
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$C\an{s[r[w]]}$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$u\simeq w \lor D$}
%     \BinaryInfC{$C\an{s[r[u]]}\lor D\uparrow s[r[w]]$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l\simeq r[u]\lor D^\prime$}
%     \BinaryInfC{$C\an{s[l]}\lor D\lor D^\prime\uparrow s[r[u]]$}
%     \DisplayProof
% \end{center}
% \rule{\textwidth}{.2pt}
% TBD.\qed



% Take the lowest \DPar inference in the tree such that it is not a \SymParG{} inference, because it was performed on the smaller side of an equality in a non-goal clause:
% \begin{center}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$s[l]\bowtie s^\prime\lor C$}
%     \AxiomC{$\dots$}
%     \noLine
%     \UnaryInfC{$l\simeq r \lor D$}
%     \BinaryInfC{$s[r]\bowtie s^\prime\lor C\lor D$}
%     \DisplayProof
% \end{center}
% \end{proof}

% % LPO with predicates assuming a precedence where predicates are greater than functions:
% % \begin{itemize}
% %     \item $p(t_1,...,t_n) \succ t$ always true by induction since base case $p(t_1,...,t_n) \succ c$ for all constants. Step case:
% %     \begin{itemize}
% %         \item $p(t_1,...,t_n) \succ x$ since $x$ cannot be instantiated to predicates.
% %         \item $p(t_1,...,t_n) \succ f(s_1,...,s_m)$ by precedence and induction hypothesis.
% %     \end{itemize}
% % \end{itemize}

% % \begin{example}

% % $$\{p(f(x)),\quad f(a)\simeq a\lor f(b)\simeq b,\quad \neg p(a)\}$$
% % How to reach $p(b)$ with only \DPar?\\
% %     \begin{prooftree}
% %         \AxiomC{$\neg p(a)$}
% %         \AxiomC{$p(f(a))$}
% %         \AxiomC{$f(b) \simeq b \lor f(a) \simeq a$}
% %         \BinaryInfC{$f(b) \simeq b \lor p(a)\downarrow p(f(a))$}
% %         \BinaryInfC{$f(b) \simeq b\downarrow p(a)$}
% %     \end{prooftree}
% % \end{example}

% \begin{example}
%     $C\an{s[r]}$ ground goal clause and $l\simeq r\lor D\lor D^\prime$ in which we can induct on something.
%     $C\an{s[l]}\lor D$
% \end{example}


==> old/intro.tex <==

Proof by induction is commonplace in modern mathematics and computational logic. Many number-theoretic arguments rely upon mathematical induction over the natural numbers, while showing correctness of software systems typically requires structural induction over inductively-defined data types, to name but two examples.
The wider automation of mathematics, logic, verification and other efforts therefore demand automated induction.\todo{add references to these two examples}

Induction can be automated by reducing goals to subgoals~\cite{ACL2,Imandra}, so that proving a goal $\forall x.F(x)$ can be proved by induction on $x$. However, splitting goals into
subgoals and organizing proof search accordingly requires expert guidance.
As an alternative, inductive reasoning has recently appeared in
SMT solvers~\cite{CVC4induction} and first-order theorem provers~\cite{CADE19,Cruanes17,Wand17}, complementing strong support
for reasoning with theories and quantifiers.
These approaches do not reduce goals to subgoals but instead implement tailored instantiations of
induction schemas\todo{cite}, adjust the underlying calculus with inductive generalizations~\cite{CICM20} and function
rewriting~\cite{FMCAD21}, and extend
theory reasoning for proving inductive
formulas~\cite{POPL17Kovacs}.

{Nevertheless, automation of induction remains  a hard problem. Even though  
a formula $\forall
x. F(x)$ is valid, it may not be provable in the underlying first-order
theory \Theory{} and calculus (see Section~\ref{motivating-example}). In particular, it may be that $\forall
x. F(x)$ is provable in \Theory{} only when \Theory{} is extended with valid first-order induction axioms; \review{by an induction axiom we mean an instance of a valid induction schema.}
%that is, instances of valid induction schemas.
We refer to the formulas
\review{used to instantiate induction schemas}
% needed to obtain such induction axioms  by instantiating the induction schemas
as \textit{auxiliary
lemmas}.}


\paragraph{\bf The Framework.} The main ingredient of this work comes with \review{weakening equational reasoning} in saturation. To this end, we introduce a set of inference rules to generate auxiliary lemmas for universally quantified goals in the unit equality setting. These inference rules generate more consequences \review{of a given goal} than the superposition calculus~\cite{DBLP:books/el/RV01/BachmairG01}, and the same consequences as general rewriting, while limiting some of the inefficiencies of the latter for \review{equational reasoning}~\cite{NieuwenhuisRubio:HandbookAR:paramodulation:2001}, in particular within the inductive reasoning context.\todo{split sentence}
\todo[inline]{We should stress that we (i) improve/enrich equality reasoning in saturation, in order to derive logical consequences that cannot be inferred using (ordered) superposition.
The benefit of using more consequences is exploited in (ii) inductive reasoning, as some of these consequences serve as auxiliary lemmas for instantiating induction schemas.
(iii) We integrate our new equality reasoning rules directly in saturation with induction...}

We integrate these rules with induction\todo{but not just induction!} directly in saturation-based first-order theorem proving~\cite{CAV13}, thus interleaving first-order theorem proving and deriving auxiliary lemmas.\todo{this suggests that these two are somehow distinct, but my understanding is that these are the same thing.}
Our approach automatically establishes the validity of Figure~\ref{fig:defs} along with many other examples, improving the state of the art in automated inductive theorem proving (Section~\ref{sec:experiments}).

\paragraph{\bf Contributions.}
To synthesize auxiliary lemmas to be used in saturation-based proof search, our work builds on rewriting for \review{equational reasoning}~\cite{NieuwenhuisRubio:HandbookAR:paramodulation:2001}. 
We embed inductive reasoning by considering valid induction schemas and adding instances of said schemas to the set of formulas to be saturated. We refer to these instances as \emph{induction axioms} and use them to prove --- and hence ensure validity of --- generated auxiliary lemmas.
% \textit{induction axioms as (candidates of) auxiliary lemmas}. 
% For example, in the motivating example from  Figure~\ref{fig:defs}(a), we use  the \textit{structural induction schema} over lists of natural numbers:
% \begin{equation}\label{eq:list-schema}
%   \big(F[\nil]\land\forall x\in\nat,y\in\lst.(F[y]\implies F[\cons(x,y)])\big)\implies \forall z\in\lst.F[z]
% \end{equation}
% and derive induction axioms from schema~\eqref{eq:list-schema} by substituting any % well-formed 
% first-order formula $F[z]$, where the $\lst$-sorted $z$ is the free variable upon which induction should be applied. 
%\lk{complete later with details on method and list of contributions}
We summarize the contributions below.
% \footnote{with proof details in the Appendix, due to space restrictions}
\begin{enumerate}[label={{\bf (\arabic*)}},wide=0em,leftmargin=0em]
    \item We introduce a simple extension of the superposition calculus, allowing us to derive formulas that could not be obtained by the \review{standard superposition} calculus. These formulas are derived during saturation as logical consequences of an input set of formulas (Section~\ref{sec:par}). We impose restrictions on \review{our calculus} to further enhance its efficiency, by \review{eliminating redundant clauses from proof search}\todo{This should be refined, maybe redundant clauses that do not serve as auxiliary lemmas either?}.\medskip

    \item We extend our calculus with tailored inductive reasoning (Section~\ref{sec:saturation}), generating auxiliary inductive lemmas as logical consequences during saturation. We also improve redundancy elimination for saturation with induction and show sufficient conditions for skipping redundant inductions and unnecessary rewrites.\medskip

    \item We implement our calculus in the \vampire theorem prover and apply it to proving inductive properties (Section~\ref{sec:impl}). We compare variants of our calculus and show that our approach improves the state of the art in \review{automation of} induction. 
\end{enumerate}

